A novel equi-dimensional finite element method for flow and transport in fractured porous media satisfying discrete maximum principle and conservation properties

Numerical simulations of flow and transport in porous media usually rely on hybrid-dimensional models, i.e., the fracture is considered as objects of a lower dimension compared to the embedding matrix. Such models are usually combined with non-conforming discretizations as they avoid the inherent difficulties associated with the generation of meshes that explicitly resolve fractures-matrix interfaces. However, non-conforming discretizations demand a more complicated coupling of different sub-models and may require special care to ensure conservative fluxes. We propose a novel approach for the simulation of flow and transport problems in fractured porous media based on an equi-dimensional representation of the fractures. The major challenge for these types of representation is the creation of meshes which resolve the several complex interfaces between the fractures and the embedding matrix. To overcome this difficulty, we employ a strategy based on adaptive mesh refinement (AMR). The idea at the base of the proposed AMR is to start from an initially uniform coarse mesh and refine the elements which have non-empty overlaps with at least one of the fractures. Iterating this process allows to create non-uniform non-conforming meshes, which do not resolve the interfaces but can approximate them with arbitrary accuracy. We demonstrate that low-order finite element (FE) discretizations on adapted meshes are globally and locally conservative and we suitably adapt an algebraic flux correction technique to ensure the discrete maximum principle. In particular, we show that the notorious conditions on M-matrices have to be adapted to the basis functions defined on non-conforming meshes. Although the proposed applications come from geophysical applications, the obtained results could be applied to any diffusion and transport problems, on both conforming and non-conforming meshes.

==> sections/02model.tex <==
\section{Mathematical and numerical problems for flow and transport problems}

In this section, we introduce the discretization on conforming meshes of the coupled models which describe the single-phase flow and the advective transport of a concentration in a fractured porous medium.
We employ models based on an \emph{equi-dimensional} representation of the fractures \cite{flemisch2018benchmarks,berre2020verification},
i.e., fractures are described as $d$-dimensional objects embedded in a $d$-dimensional porous matrix.
We also introduce the relevant properties of the two discretizations in term of discrete maximum principle, positivity of the solution, and conservation.
In the next sections, we will extend these concepts to non-conforming meshes.

%From an abstract point of view, the flow problem is a Laplace interface problem with piecewise constant permeability.


\subsection{Preliminaries definitions}
\label{sub:matpre}

We denote by $\domain$ an axis-aligned box domain in $\mathbb R^d$,
where $d$ denotes the dimension of the problem.
The length along the $i$-axis is denoted by $L_i$.
We denote by $\partial \domain$ the boundary of $\domain$.
The outward unit vector to $\domain$ is denoted by $\mvecfun n$.
Points of $\domain$ will be denoted by capital non-bold letters $X$ and their coordinates by $\mpoint {x}=(x_1,x_2, \ldots, x_d)$.

Over $\domain$, we introduce a set $\fracset$ of $d$-dimensional inclusions $f_i \subset \domain$ with $i=1,2\,\ldots \cardfracset$,
where $\cardfracset= | \fracset |$ is the number of inclusions.
Inclusions are non axis-aligned boxes, i.e., rectangles for $d=2$ or cuboids for $d=3$.
We are in particular interested to the case where inclusions have one dimension that is much smaller compared to the other(s).
In this case, we will refer to such inclusions as fractures and the smaller dimension will be referred to as aperture or thickness.

We define $\domain_f:=\bigcup_{i=1}^{\cardfracset}f_i$, i.e., the sets of the inclusions and $\domain_m := \domain \backslash \domain_f$, i.e., the set representing the matrix.
Both $\Omega_m$ and $\Omega_f$ may be non-connected sets.
The set $\Gamma:= \overline \Omega_m \cap \overline \Omega_f$ is the interface between the two subdomains.

We denote the fracture aperture by $w$, the permeability by $k$, and the porosity by $\phi$.
Permeability and porosity are assumed to be real functions attaining constant positive values over $\Omega_m$ and $\Omega_f$,
such as, for example,
\begin{equation}
k=\begin{cases} k_m, \quad \text{ in } \domain_m,\\
k_f, \,\,\quad \text{ in } \domain_f.\\
\end{cases}
\end{equation}

It is worth to point out that the assumptions adopted to introduce the reader to the topic could be relaxed:
$\domain$ has not to be a box domain;
fractures may have a variable apertures and  different shapes; the material properties can be heterogeneous. In particular, heterogenous properties would require to replace scalar values by tensor quantities.

We suppose that $\partial \domain$ can be decomposed in two subsets $\dirset$ and $\neuset$
with $\partial \Omega=\cdirset \cup \cneuset $ and $\idirset \cap \ineuset = \emptyset$.
For each of the problems, the set $\dirset$ denotes the subset of $\partial \domain$ where Dirichlet boundary conditions are imposed.
$\dirset$ may differ for flow and transport problems.

We use the standard notation $H^s(\domain)$ to denote the Sobolev space based on $L^2(\domain)$.
The space $H^s(\domain)$ is endowed with the usual norm $\| \, \cdot \, \|_s$, semi-norm $| \, \cdot \, |_s$, and scalar product $(\,\cdot\,,\, \cdot \, )_s$.
%$H^1_{\dirset} (\domain)=\{ v \in H^1(\domain) \, : \, v|_S=0 \}.$

For an unknown $q$ and Dirichlet boundary conditions $q_D$ imposed on $\dirset$,
for each of the problems, the set $\mS$ denotes a suitable function space where the solution is sought.
Moreover, we define the function set
\begin{equation}
\mU=\{ v \in \mS \, : \, v=q_D \text{ on } \dirset\}
\end{equation}
and the function space
\begin{equation}
\mV=\{ v \in \mS \, : \, v=0 \text{ on } \dirset\}.
\end{equation}
 
%We introduce a mesh over $\domain$, i.e., a partition into closed elements $E$ such as
%$$\mesh= \big\{  E \subset \domain \, : \,  \bigcup {E} = \domain \,\,\text{and}\,\, \mathring{E}_i \cap \mathring{E}_j = \emptyset \,\, \text{for} \,\, i\neq j \big\}.$$
%Elements can be triangles or quadrilaterals for $d=2$ and tetrahedra or hexahedra for $d=3$.
%We assume that all elements of a mesh are of the same type.
Over $\domain$, we introduce a mesh $\mesh$ with $N_E$ elements and $N_N$ nodes.
%$$\mesh= \big\{  E \subset \domain \, : \,  \bigcup {E} = \domain \,\,\text{and}\,\, \mathring{E}_i \cap \mathring{E}_j = \emptyset \,\, \text{for} \,\, i\neq j \big\}.$$
Elements can be triangles or quadrilaterals for $d=2$ and tetrahedra or hexahedra for $d=3$.
We assume that all elements of a mesh are of the same type.
Elements are denoted by $E$ andf
have vertices, edges, and, for $d=3$, faces.
The term side refers to edges for $d=2$ and to faces for $d=3$.
We assume, for now, that the mesh is conforming, i.e., 
the intersection of each pair of elements is empty, a vertex, an edge, or a face.


We let $\hh{\mS}$ denote the nodal interpolation space over $\mesh$, i.e.,
$$\hh{\mS}= \{ v \in C^0 (\Omega) \, : \, v |_E  \in \mathbb L_1 \},$$
where $\mathbb L_1$ is the space of linear functions on $E$ for triangular and tetrahedral meshes (usually denoted by $\mathbb P_1$)
or the space of multi-linear functions on $E$ for quadrilateral or hexahedral meshes (usually denoted by $\mathbb Q_1$).

We let $\iset$ denote the set of all nodal indices $A = 1, 2, \ldots , n_{np}$ and
we let $\isetdir$ be the subset corresponding to nodes located in $\dirset$, i.e.,
$$\isetdir = \{ A \, : \, \mpoint{x}_A \in \dirset \},$$
and $\isetrest = \iset \setminus \isetdir$.
We call $\mb{A}$ the basis function associated to the node $\mpoint{x}_A$.
Observe that the space $\hh{\mS}= \mathrm{span}\{ \mb{A}\}_{A\in \iset}$.

We denote the set of functions in $\hh{\mS}$ which satisfy the Dirichlet boundary condition as $\hh{\mU}$ and
the set of functions $\hh{\mS}$ which attain zero value on the Dirichlet boundary as $\hh{\mV}$.
Finally, we introduce $\hh{\mG} = \mathrm{span}\{\mb{A}\}_{A \in \isetdir}$, i.e.,
the span of the basis functions associated with the set of nodes in $\isetdir$.
We observe that the space $\hh{\mV}$ is the span of the basis functions associated with each node except the ones where Dirichlet conditions are imposed,
and the following relations hold:
\begin{equation}
\begin{array}{lcll l}
\hh{\mU} &= & \mU \cap \hh{\mS},\\
\hh{\mV} &= & \mV \cap \hh{\mS}  &= &  \mathrm{span}\{ \mb{A}\}_{A\in \isetrest},\\
\hh{\mS} &= & \hh{\mV} \bigoplus \hh{\mG} &= &  \mathrm{span}\{ \mb{A}\}_{A\in \iset},\\
\hh{\mU} &\subset& \hh{\mS}.
\end{array}
\end{equation}


\subsection{The flow problem}

For an incompressible single-phase fluid, the flow through a porous medium is described by
\begin{equation}
\label{eq:flowstrong}
\begin{array}{c c c l}
\nabla \cdot \mvecfun{u} &= & 0 & \quad \text{in } \domain,\\
\mvecfun{u} &= & -k \nabla p & \quad \text{in } \domain,\\
 p & = &  g & \quad \text{on} \,\, \dirset,\\
 k \nabla p \cdot \mvecfun n& = &  h & \quad \text{on} \,\, \neuset,
\end{array}
\end{equation}
where $\mvecfun{u}$ is the velocity and $p$ the pressure.
For the flow problem, we set $\mU=\{ v \in H^1(\domain) \, : \, v|_{\dirset}=g\}$
and $\mV = H^1_{\dirset} (\domain)$.
The weak formulation of problem \eqref{eq:flowstrong}
\begin{equation}
\label{eq:flowweak}
%\boxed{
\begin{array}{l}
\text{Find } p\in U \, \text{ such that }\\[2mm]
{\displaystyle d(p,v) = f(v) \quad \forall v \in V,}
\end{array}
%}
\end{equation}
where
$$d(p,v)= \int_\domain k\, \nabla p \cdot \nabla q \,\text{d}V  \quad \text{and} \quad f(v)=  \int_{\neuset} h \, v  \,\text{d}A.$$
%
%Existence, uniqueness, and stability results for the problem above follow from Lax-Milgram theorem.
%As the permeability is discontinuous, the flow problem is an interface problems.
%The presence of the interface limits the regularity of solution of the problem.
%Actually, being $k$ bounded from below and above,
%theorem 6.1 of \cite{petzoldt} can be applied,
%hence the following result holds.
%
%\begin{mytheo}
%The solution of problem \eqref{eq:flowweak} fulfils $u \in H^{1+1/4}(\Omega)$.
%\end{mytheo}
%
%Moreover, as we allow to have mixed boundary conditions,
%on the boundary there may exist homogeneous singular points, i.e.,
%points where the type of boundary conditions changes.
%Close to singular points, the solution can be written as the sum of a regular function and a finite number of singular functions whose number and regularity depend on the size of the angle at the singular point \cite{grisvard,mgzhali}.
%Hence, due to discontinuities of $k$ and the presence of singular points,
%the solution $u$ may not have the optimal $H^2$ regularity which could be naively supposed for a problem with a load function $0$.
%%Regularity is fundamental in the application of discretization methods, as it allows to obtain the theoretical convergence results.
%The flow problem  satisfis the maximum principle \cite{kuzmin}.

\begin{mytheo}
The following a-priori estimates hold for problem~\eqref{eq:flowweak}:
\begin{align}
\min_{\partial \domain} p < p<\max_{\partial \domain}   p & \qquad \quad (\text{Maximum Principle}), \label{eq:contmp} \\
p|_{\partial \domain}\geq0 \implies p\geq 0 & \qquad \quad  \text{(Positivity preservation)} \label{eq:contposotivity}.
\end{align}
\end{mytheo}


With the definitions introduced in Subsection \ref{sub:matpre},
the finite element approximation to problem~\eqref{eq:flowstrong} reads
\begin{equation}
\label{eq:flowweakdiscrete}
%\boxed{
\begin{array}{l}
\text{Find } \hh{p} \in \hh{U} \, \text{ such that }\\[2mm]
{\displaystyle d( \hh{p}, \hh{v}) = f( \hh{v}) \quad \forall \hh{v} \in \hh{V},}
\end{array}
%}
\end{equation}
where
$$ d( \hh{p}, \hh{v}) = \int_\domain k\, \nabla p_h \cdot \nabla v_h \,\text{d}V  \quad \text{and} \quad f(v)=  \int_{\neuset} h \, v _h \,\text{d}A.$$

Hence, the flow prolem admits the following algebraic representation
\begin{equation}
\label{eq:flowdiscrete}
\mathbf D\\
\mathbf p\\
=
\mathbf f,
\end{equation}
or

\begin{equation}
\label{eq:flowdiscrete2}
\begin{pmatrix}
\mathbf D_{II} & \mathbf D_{ID} \\
\mathbf 0 & \mathbf I
\end{pmatrix}
\begin{pmatrix}
\mathbf p_{A} \\
\mathbf p_D 
\end{pmatrix}
=
\begin{pmatrix}
\mathbf f_{A} \\
\mathbf g_D 
\end{pmatrix},
\end{equation}
where
\begin{equation*}
\begin{array}{l c l  c  l}
\matent{D_{II}}{A}{B} & = &d(\mb{B},\mb{A}) &  \quad & A,B\in \isetrest,\\
\matent{D_{ID}}{A}{B} & =& d(\mb{B},\mb{A}) &  \quad & A\in \isetrest, \, B \in \isetdir,\\
\matent{f_{A}}{A}{} & =& f(\mb{A}) &  \quad & A\in \isetrest.\\
\end{array}
\end{equation*}
We introduce the total flux $\mflux{\domain}{\dirset}$ along the Dirichlet boundary $\Gamma_D$, and restate Problem~\eqref{eq:flowweakdiscrete} as follows:
\begin{equation}
\label{eq:auxflow_global}
%\boxed{
\begin{array}{l}
\text{Find}\,\, (\hh{u} , \mflux{\domain}{\dirset}) \in \hh{U}\times \hh{G}\,\,\text{such that}\\[2mm]
{\displaystyle d( \hh{p}, \hh{v}) +(\mflux{\domain}{\dirset} ,\hh{v})_{\dirset} = f( \hh{v})  \quad\forall \hh{v}\in \hh{\mS} }
\end{array}
%}
\end{equation}
where $(\cdot,\cdot)_{\dirset}$  is the $L^2$ scalar product over $\dirset$. Setting $v_h=1$ into the above equation shows that $\mflux{\domain}{\dirset}$ is globally conservative:
$$ \int_{\Gamma_D}\mathcal{F}_D^h(\Omega)\,d\text{A} + \int_{\Gamma_N} h  \,\text{d}A=0$$
%which proves that the continuous Galerkin formulation is globally conservative.
% $\mflux{\domain}{\dirset}$ represents the flux across the boundary $\dirset$ and
Formulation~\eqref{eq:auxflow_global} can be split into two sub-problems:\\
$\text{Find}\,\, (\hh{u} , \mflux{\domain}{\dirset}) \in \hh{U}\times \hh{G}\,\,\text{such that}$
\begin{align}
\label{eq:auxflow_global_split_a}
d( \hh{p}, \hh{v}) &= f( \hh{v}) & \forall \hh{v} \in \hh{V},\\
\label{eq:auxflow_global_split_b}
(\mflux{\domain}{\dirset} ,\hh{v})_{\dirset} &=d( \hh{p}, \hh{v}) - f( \hh{v}) & \forall \hh{v}\in \hh{G}.
\end{align}
which admit the following algebraic representation:
\begin{equation}
\label{eq:flowdiscretehughes}
\begin{pmatrix}
\mathbf D_{II} & 0 \\
-\mathbf D_{ID} & \mathbf M_{B}
\end{pmatrix}
\begin{pmatrix}
\mathbf p_{A} \\
\mathbf h_D 
\end{pmatrix}
=
\begin{pmatrix}
\mathbf f_{A} -  \mathbf D_{ID}  \mathbf g_D \\
-\mathbf f_D 
\end{pmatrix},
\end{equation}
Here  $\mathbf M_{B}$ is the boundary mass matrix assembled on $\Gamma_D$ and
\begin{equation*}
\begin{array}{l c l  c  l}
\matent{D_{II}}{A}{B} & = &d(\mb{B},\mb{A}) &  \quad & A,B\in \isetrest,\\
\matent{D_{ID}}{A}{B} & =& d(\mb{B},\mb{A}) &  \quad & A\in \isetrest, \, B \in \isetdir,\\
\matent{f_{A}}{A}{} & =& f(\mb{A}) &  \quad & A\in \isetrest.\\
\end{array}
\end{equation*} 
From the second row of \eqref{eq:flowdiscretehughes} it follows that the evaluation of the boundary flux is \textit{post-processing} calculation requiring the inversion of the matrix $\mathbf M_{B}$.


\subsection{The transport problem}

The transport problem is coupled to the flow problem through the velocity $\mvecfun u$ as it enters both in the definition of the boundary conditions
and in the transport equation.
We let $\Gamma_{in} := \{ \mathbf x \in \partial \Omega \, : \,  \mvecfun u \cdot \mvecfun n < 0\}$ denote the inflow boundary
and $\Gamma_{out} := \{ \mathbf  x \in \partial \Omega \, : \,  \mvecfun u \cdot \mvecfun n \geq 0\}$ denote the outflow boundary.
The unknown is a concentration $c=c(\mathbf x, t)$.
The equi-dimensional model for the advective transport problem reads:

\begin{equation}
\label{eq:flowclassic}
\left\{
\begin{array}{r c l l}
{\displaystyle \phi \frac{\partial c}{\partial t} +  \nabla \cdot ( \mvecfun u \, c ) }& = &0 &\quad \text{in}\,\, \Omega \times \mathscr I\\
c( \,\cdot \, , 0) &= & c_0 &  \quad \text{in}\,\, \Omega\\
c & = & c_D & \quad \text{on}\,\, \Gamma_{in} \times \mathscr I
\end{array}
\right.
\end{equation}
Here, $\mathscr I=(0, T_{\text{fin}}]$ is the time interval, $c_0$ is the initial condition, and
$c_D$ is the inflow Dirichlet boundary condition.

Defining by $\Sigma$ the set of points where initial and boundary conditions are prescribed, i.e., 
$$\Sigma:=\{(\mathbf x,t) \, : \, \mathbf x \in \Gamma_{in} \lor t = 0\},$$
the following theorem holds.
\begin{mytheo}
\label{theo:this}
For problem \eqref{eq:flowclassic} the following a-priori estimates hold:
\begin{equation*}
\begin{array}{r c l l}
\nabla \cdot \mvecfun u=0&\implies &\min_{ \Sigma} c \leq c\leq \max_{ \Sigma}  c& \quad(\text{Maximum Principle}) \\[1mm]
c|_{\Sigma}\geq0&\implies & c\geq 0 & \quad\text{(Positivity preservation)}
\end{array}
\end{equation*}
\end{mytheo}

%\begin{mytheo}
%\label{theo:this}
%For problem \eqref{eq:flowclassic} the following a-priori estimates hold:
%\begin{align}
%\nabla \cdot \mathbf{u}=0&\implies &\min_{ \Sigma} u \leq u\leq \max_{ \Sigma} u.\quad(\text{Maximum Principle}),\\
%u_{\Sigma}\geq0&\implies & u\geq 0\quad\quad\quad\quad\quad\quad\quad\text{(Positivity preservation)}.
%\end{align}
%\end{mytheo}
Theorem \ref{theo:this} ensures that if $c_0$ and $g$ are positive,
then the solution is positive all over the space-time domain.
Moreover, the solution in the domain cannot exceed the maximum value injected in the inflow boundary.



\subsubsection*{Finite element discretization of transport equation}

The function $c_h=c_h(\, \cdot \, , t) \in U_h$ is the approximation of  the concentration $c$ at time $t$
and $\mathbf c(t)$ is the time dependent array having as components the unknown coefficients $c_j$ with respect to the basis $\{ N_j \}$.
The spatial discretization of \eqref{eq:flowclassic} reads:
\begin{equation}
\label{eq:transportweakdiscrete}
%\boxed{
\begin{array}{l}
\text{For all } t \in \mathscr I, \text{ find } c_h(\, \cdot \, , t) \in U_h \, \text{ such that } c( \,\cdot \, , 0) =  c_0,\,\, \text{and} \\[2mm]
{\displaystyle m \left( \dfrac{ \partial c_h}{\partial t} , q_h \right ) + a (c_h , q_h)= 0 \quad \forall q_h \in V_h.}
\end{array}
%}
\end{equation}
where  we have used the following discrete bilinear forms
\begin{equation}
\nonumber
\begin{array}{ l c l}
 m \left( \dfrac{ \partial c_h}{\partial t} , q_h \right ) &=& {\displaystyle \hphantom{-} \int_\Omega \phi \, \dfrac{ \partial c_h}{\partial t}  \, q_h \, \text{d}V}\\[3mm]
 \nonumber
 a (c_h , q_h) & = & {\displaystyle - \int_{\Omega} c_h\, \mvecfun u\cdot \nabla q_h \,\text{d}V + \int_{\Gamma_{out}} c_h \, q_h \, \mvecfun u \cdot \mvecfun n \,\text{d}A }
\end{array}
\end{equation}
Problem \eqref{eq:transportweakdiscrete} admits the following algebraic representation
\begin{equation}
\label{eq:flowdiscrete}
\mathbf M \frac{ \text{d} \mathbf c }{ \text{d} t} + \mathbf A \mathbf c = \mathbf 0.
\end{equation}
In case of conforming meshes and discretizations,
the entries of the mass matrix $\mathbf M$ and of the discrete transport operator $\mathbf A$ are computed as:
$$\matent{M}{A}{B}=m( N_B ,N_A)  \text{\,\,\,and\,\,\,} \matent{A}{A}{B}=a( N_B ,N_A) .$$
%, where  $\{N_k\}_{k\in J^T}$ and suitable basis functions and $J^T$ i an index set.

The following theorem provides sufficient conditions 
to have the maximum principle and positivity preservation for the semi-discrete transport problem~\eqref{eq:flowdiscrete}.
\begin{mytheo}
\label{th:DM}
\text{Suppose that}:
$$\matent{M}{A}{A} > 0, \,\,\, \matent{M}{A}{B}= 0, \,\,\, \matent{A}{A}{B}  \leq 0, \,\,\, \forall B \neq A.$$

Then the following a priori estimates hold for the coefficient $c_A$:
\begin{itemize}
\item [1a] The {semi-Discrete Maximum Principle} (DMP) is satisfied:

$\quad\quad{\displaystyle \sum_{B}\matent{A}{A}{B}=0, \quad  c_B\geq c_A, \quad \forall B \neq A \quad  \implies \quad \dfrac{d c_A}{dt} \leq 0.}$
\item [1b] The {positivity preservation} is satisfied:  $$c_B(0) \geq 0,\, \forall B\,\, \,\,\implies c_A(t)\geq0, \forall t>0.$$
\end{itemize}
\end{mytheo}


Continuous finite element discretizations applied to transport problems are characterized by spurious undershoots and overshoots in the numerical solution
as they do not satisfy satisfy the hypothesis of theorem~\eqref{th:DM}.
Several \emph{stabilization} strategies have been proposed
%with some of them working either on  the Galerkin formulation or on the algebraic representation
with the goal of making $\mathbf M$ and $\mathbf A$ consistent with the hypotheses of the theorem.
In the next, we refer to the flux corrected transport scheme proposed by \cite{Kuzmin}.
The basic idea of this method is introduce discrete diffusion operators
that allow to preserve of positivity of the solution and ensure the DMP.


The fully discrete counterpart of problem \eqref{eq:flowdiscrete} is
\begin{equation}
\label{eq:flowweakalg}
 \mathbf M\\
\mathbf c^{n+1}+\Delta t\mathbf A \mathbf{c}^{n+1}\\
=\mathbf M \mathbf c^{n}
\end{equation}
where an implicit Euler time stepping scheme has been adopted for the temporal discretization, and the time-step size is denoted by $\Delta t$.
We point out that the backward Euler scheme is strongly stable with no restriction on the time-step size $\Delta t$~\cite{nmdp}.

%\subsubsection*{Stabilization of the  transport problem}
%
%(TRASH FROM PREVIOUS SECTION)
%~\\
%~\\
%For the numerical approximation of problem \eqref{eq:flowclassic}, we have to introduce temporal and spatial discretization.
%
%For the temporal discretization,
%we employ a an implicit Euler approximation method.
%We divide $\mathscr I$ into intervals of size $\Delta t$ and we let $t_i=i\, \Delta t$.
%We define $c^n(\mathbf x)$ the approximation to $c(\mathbf x, t^i)$.
%
%Hence, at each step $n+1$ we deal with the problem
%\begin{equation}
%\label{eq:flowclassicdt}
%\left\{
%\begin{array}{r c l l}
%{\displaystyle \phi c^{n+1} + \Delta t\,  \nabla \cdot ( \mvecfun u \, c^{n+1} ) }& = &\displaystyle \phi c^{A} &\quad \text{in}\,\, \Omega \\
%c & = & c_D & \quad \text{on}\,\, \Gamma_{in}.
%\end{array}
%\right.
%\end{equation}
%
%
%Let  $U(_h\mathcal T)$ be the finite element space defined as $ U_h(\mathcal T) = H^1_{\Gamma_in}(\Omega) \cap X(\mathscr T)$ and $V(\mathcal T) = H_{0}^1(\Omega) \cap  X(\mathcal T)$, then the  Galerkin approximation of the transport problem reads as:
%\begin{equation}
%\label{eq:flowweakdiscrete}
%%\boxed{
%\begin{array}{l}
%\text{Find } c_h^{i+1}\in U_h(\mathcal T) \, \text{ such that }  \forall q_h \in V_h(\mathcal T )\\[2mm]
%{\displaystyle \int_\Omega \phi\, c_h^{n+1} \, q_h \,\text{d}V -\Delta t \int_{\Omega} c_h^{n+1} \mvecfun u \cdot \nabla q_h \,\text{d}V + \int_{\Gamma_{out}} c_h^{n+1} q_h \mvecfun u \cdot \mvecfun n \,\text{d}A  = \int_\Omega \phi\, c_h^{n} \, q_h \,\text{d}V.}
%\end{array}
%%}
%\end{equation}
%
%After introducing suitable basis functions $\{N^a_i\}_{i\in J^T}$, with $J^T$ being an index set, the discretized problem \eqref{eq:flowweakdiscrete} admits the following algebraic representation
%~\\
%~\\
%(END TRASH)

\subsubsection*{Flux corrected transport}

We adopt a flux corrected transport (FCT) method to satisfy the assumptions of theorem~\eqref{th:DM}, and thus preserving the positivity/monotonicity of the solution for the transport problem~$\eqref{eq:flowweakdiscrete}$ by suppressing the presence of under/overshoots.

The FCT methodology is a predictor-corrector strategy which consists of two main steps:
\begin{itemize}
\item Step 1. Advance the solution in time by a low-order scheme that incorporates enough numerical diffusion to suppress undershoots
and overshoots.
\item Step 2. Correct the solution using antidiffusive fluxes limited in such a way that no new maxima or minima can form and existing
extrema cannot grow.
\end{itemize}
To satisfy the hypothesis of theorem~\ref{th:DM}, one needs to approximate the consistent mass matrix $\mathbf M$ by its lumped counterpart $\mathbf{M}_L$ and eliminate the off diagonal positive entries of the transport operator $\mathbf{A}$ by adding a  discrete diffusion contribution defined such that $ \matent{A}{A}{B}+ \matent{A_s}{A}{B}\leq0$:
$$ \matent{A_s}{A}{B}=-\,\max(0,  \matent{A}{A}{B},  \matent{A}{B}{A})\quad  \matent{A_s}{A}{B}=-\sum_{B=1,B \neq A}^{N}  \matent{A_s}{A}{B}$$
where $N$ is the number of degrees of freedom of the problem.

In the process of algebraic flux correction, the discrete problem ~\eqref{eq:flowweakalg} can be split into a \textit{good} diffusive part of the form
$$\mathbf{M}_L \mathbf{c}^{n+1} +(\mathbf{A} +  \mathbf{A}_s)\,\mathbf{c}^{n+1}\, \Delta t=\mathbf M_L \mathbf c^{n}$$

where the matrix $\matent{A_s}{A}{B}$  is the artificial diffusion operator, and a \textit{bad} anti-diffusive part given by:
$$\mathbf{f}=(\mathbf{M}_L-\mathbf{M})\mathbf{c}^{n+1} + \mathbf{A}_s\mathbf{c}^{n+1} \,\Delta t - (\mathbf{M}_L - \mathbf{M})\mathbf{c}^{n}$$

Indeed the \textit{good} diffusive counter is positivity-preserving but overly diffusive due to its linearity. Hence, a nonlinear antidiffusive correction is required to recover the accuracy of the original high-order discretization.

The bad anti-diffusive term admits the decomposition $[\mathbf{f}]_A=\sum_{B\neq A}\matent{f}{A}{B}$ where the components of the sums satisfy property  $\matent{f}{A}{B}+\matent{f}{B}{A}=0$  and describe the numerical flux from $B$ to node $A$:

$$ \matent{F}{A}{B}=\matent{M}{A}{B}(\mathbf{c}^{n+1}_{A}-\mathbf{c}_B^{n+1})- \matent{M}{A}{B}(\mathbf{c}^{n}_{A}-\mathbf{c}_B^{n})-\matent{D}{A}{B}(\mathbf{c}^{n+1}_{A}-\mathbf{c}_B^{n+1})\,\Delta t $$

For  ensuring the positivity of the solution, every anti-diffusive flux $\matent{F}{A}{B}$ is multiplied by a solution-dependent correction factor
 $0\leq\alpha\leq 1$ such that the flux-corrected discrete scheme reads:
$$\mathbf{M}_L \mathbf{c}^{n+1} + \Delta t(\mathbf{A} +  \mathbf{A}_s)\,\mathbf{c}^{n+1}=\mathbf M_L \mathbf c^{n} + \widetilde{\mathbf{f}}$$
with $[\widetilde{\mathbf{f}}]_A= \sum_{B\neq A} \matent{F}{A}{B}\matent{{\alpha}}{A}{B}$.
By definition, the high-order discretization is recovered for $\matent{\alpha}{A}{B}=1$, and the lower discretization is attanied for $\matent{\alpha}{A}{B}=0$. The resulting FCT scheme is summerized in algorithm~\ref{algo:FCT}.

\begin{figure}[ht!]
\begin{algorithm}[H]
% \KwData{this text}
\textbf{Step 1}. \\
Advance in time by solving for the system:

$$[{\mathbf{M}_L } + {\Delta t}(\mathbf{A} + \mathbf{A}_s)]\mathbf{c}^{L}={\mathbf{M}_L}\mathbf{c}^{n}$$

\textbf{Step 2}\\
Correct the solution using anti-diffusive fluxes: % limited .

$$\matent{F}{A}{B}=\matent{M}{A}{B}(\dot{\mathbf{c}}_B^L-\dot{\mathbf{c}}_A^L) + \matent{A_s}{A}{B}(\mathbf{c}_{A}^L-\mathbf{c}_{B}^L),\,\, \text{with} \,\,B\neq A $$
where $ \dot{\mathbf{c}}^L$ is defined as: $\dot{\mathbf{c}}^L=\mathbf{M}_L^{-1}\mathbf{A}_s\mathbf{c}^L$.\\
\vspace{0.2cm}
\textbf{Step 3}\\
Limit $\matent{F}{A}{B}$ in such a way that the discrete maximum principle is preserved:
$$[\widetilde{\mathbf{f}}]_A=\sum_{B\neq A}\matent{\alpha}{A}{B}\matent{f}{A}{B}\,\,\quad 0\leq \matent{\alpha}{A}{B} \leq 1$$

\textbf{Step 4}\\
Compute the final solution as:
$$\textbf{M}_L\textbf{c}^{n+1}=\textbf{M}_L\textbf{c}^{L}+ \Delta t~\widetilde{\mathbf{f}}$$
\end{algorithm}
 \caption{Algorithm to stabilize the Transport problem.}
 \label{algo:FCT}
\end{figure}

Several approaches have been proposed to quantify the value of the limiting coefficients $\alpha_{A}{B}$. In particular, we employ the Zalesak’s fully multidimensional FCT algorithm proposed in~\cite{Kuzmin} which ensures that anti-diffusive fluxes do not cause the nodal solution $[\mathbf{c}]_A$ to exceed some maximum $\mathbf{c}_{max}$ value or fall below some
minimum value  $\mathbf{c}_{min}$ depending on the boundary conditions.


%The \text{flux corrected counterpart} of (1) is a semi-discrete problem:
%$$\mathbf{M}_L\dfrac{d \mathbf{c}}{dt} + (\mathbf{A} +  \mathbf{D})\,\mathbf{c } = \widehat{\mathbf{f}}$$
%with $\widehat{f}_i=\sum_{B\neq A}\alpha_{A}{B}f{A}{B}$ and $0\leq \alpha_{B}{A} \leq 1$
%In the absence of a second order term, boundary conditions cannot be imposed on the outflow boundary.
%We define the set
%$$U=\{ v \in H^1(\Omega)\, : \,  u|_{\Gamma_{in}}=c_D \}$$
%and the function space
%$$V=\{ v \in H^1(\Omega)\, : \,  u|_{\Gamma_{in}}=0 \}.$$
%For the transport problem, we can define the following weak problem:


%\begin{equation}
%\label{eq:flowweakdiscrete}
%%\boxed{
%\begin{array}{l}
%\forall t \in \mathscr I, \text{find } c \in U \, \text{ such that }\\[2mm]
%{\displaystyle \int_\Omega \phi \frac{\partial c}{\partial t}  q \, \text{d}V - \int_{\Omega} c \mvecfun u \cdot \nabla q \,\text{d}V + \int_{\Gamma_{out}} c\, q\, \mvecfun u \cdot \mvecfun n \,\text{d}A  = 0 \quad \forall q \in V.}
%\end{array}
%%}
%\end{equation}

%(TROVARE QUALCUNO CHE FA L'ANALISI DI QUESTO TIPO DI PROBLEMA, VEDI AD ES. HUGHES 2000 PER IL CASO STAZIONARIO.)



% Equazione generica ellittica + time derivative Principio del massimo,


==> sections/04conservation_mio.tex <==
\section{Conservation properties of continuous finite element methods}
\label{sec:conservation}
In this section, we derive the global and local conservation properties of FE discretizations on non-conforming meshes. 
We refer to a diffusion problem, such as the flow one, but they can be equally proven for all the cases considered in~\cite{hughes}.
The idea at the base of the proofs is that the basis functions form a partition of unity, i.e., they sum of the evaluation of all the basis functions at a point $\mathbf x$ is one.
Equivalently, we can observe that the function one belongs to the space of the  test functions or that row-sum of the stiffness matrix is zero.

While the proof of the global conservation properties is identical to the case on conforming meshes,
the main difference in the proof of the local conservation properties is in the definition of suitable spaces of test functions.
The use of this definition allows to show that the FE method is conservative also between subsets that do not coincide with some elements of the mesh.

\paragraph{Global conservation properties}

We assume that the function spaces defined in Eq.~\eqref{eq:discretespacedefinition} are built on a conforming mesh and spanned by the functions $\mbconf{i}$.
In order to show the global conservation, we introduce the approximated flux $\mflux{\domain}{D}$ along the Dirichlet boundary $\Gamma_D$, and restate Problem~\eqref{eq:flowweakdiscrete} as follows:
\begin{equation}
\label{eq:auxflow_global}
%\boxed{
\begin{array}{l}
\text{Find}\,\, (\hh{u} , \mflux{\domain}{D}) \in \hh{U}\times \hh{G}\,\,\text{such that}\\[2mm]
{\displaystyle d( \hh{p}, \hh{v}) +(\mflux{\domain}{D} ,\hh{v})_{D} = f( \hh{v})  \quad\forall \hh{v}\in \hh{\mS} }.
\end{array}
%}
\end{equation}
Setting $\hh{v}=1$ into the above equation, we obtain
$$ \int_{\Gamma_D}\mflux{\domain}{D}\,\text{d}{\Gamma} + \int_{\Gamma_N} h  \,\text{d}\Gamma=0.$$
This shows that that $\mflux{\domain}{D}$ is the flux associated to the Dirichlet boundary conditions and makes the method globally conservative.

Formulation~\eqref{eq:auxflow_global} can be split into two sub-problems:\\
$\text{Find}\,\, (\hh{u} , \mflux{\domain}{D}) \in \hh{U}\times \hh{G}\,\,\text{such that}$
\begin{align}
\label{eq:auxflow_global_split_a}
d( \hh{p}, \hh{v}) - f( \hh{v})&=0 & \forall \hh{v} \in \hh{V},\\
\label{eq:auxflow_global_split_b}
(\mflux{\domain}{D} ,\hh{v})_{D} &= d( \hh{p}, \hh{v}) - f( \hh{v}) & \forall \hh{v}\in \hh{G}.
\end{align}
which admit the following algebraic representation:
\begin{equation}
\label{eq:flowdiscretehughes}
\begin{pmatrix}
\mathbf D_{II} & 0 \\
-\mathbf D_{ID} & \mathbf B_{DD}
\end{pmatrix}
\begin{pmatrix}
\mathbf p_{I} \\
\mathbf h_D 
\end{pmatrix}
=
\begin{pmatrix}
\mathbf f_{I} -  \mathbf D_{ID}  \mathbf g_D \\
-\mathbf f_D 
\end{pmatrix},
\end{equation}
Here  $\mathbf B_{DD}$ is the boundary mass matrix on $\Gamma_D$ and
\begin{equation*}
\begin{array}{l c l  c  l}
\matent{D_{II}}{i}{j} & = &d(\mb{B},\mb{i}) &  \quad & i,j\in \isetrest,\\
\matent{D_{ID}}{i}{j} & =& d(\mb{B},\mb{i}) &  \quad & i\in \isetrest, \, j \in \isetdir,\\
\matent{f_{I}}{i}{} & =& f(\mb{i}) &  \quad & A\in \isetrest.\\
\end{array}
\end{equation*} 
From \eqref{eq:auxflow_global_split_b} or, equivalently, the second row of \eqref{eq:flowdiscretehughes},
we notice that the computation of the boundary flux associated to $\Gamma_D$ requires the inversion of the boundary mass matrix $\mathbf B_{DD}$,
which can be thought as a \textit{post-processing} evaluation.


%Again, the space $V^r$ is the span of the basis functions associated with each node except the ones where Dirichlet conditions are imposed, and the following equalities hold:


%\begin{equation}
%\begin{array}{lcll l}
%G^r&=&\mathrm{span}\{N_A^r\}_{D}\\
%U^h &= & U \cap S^h,\\
%V^r &= &V \cap S^h  &= &  \mathrm{span}\{ \mb{i}\}_{A\in I},\\
%S^h &= &V^r \bigoplus G^r &= &  \mathrm{span}\{ \mb{i}\}_{A\in \isetreg},\\
%U^h &\subset& S^h.
%\end{array}
%\end{equation}

\paragraph{Local conservation properties}

Let $\domain_1 \subset \domain$  and $\domain_2 \subset \domain$  be two non-overlapping subdomains such that $\overline{\domain}_1\cup \overline{\domain}_2= \overline{\domain}$.
We denote the boundary of the subdomain $\domain_1$ by $\Gamma_1$,
the boundary of the subdomain $\domain_2$ by $\Gamma_2$,
and the interface between the $\domain_1$ and $\domain_2$ (i.e., $\Gamma_1 \cap \Gamma_2$) by $L$ .
The subdomain $\domain_1$ could either be interior to $\domain$
or intersect the boundary of  $\domain$ in either a finite number of isolated points or a set with finite measure.

For the sake of simplicity, we assume that $\Gamma_1$ only overlaps with the Neumann boundary $\Gamma_N$ and denote by $\Gamma_1^N=\Gamma_1\cap\Gamma^N$ their intersection such that $\Gamma_1=L \cup \Gamma_1^N$. In the same way, the boundary $\Gamma_2\setminus L$ is split into the Neumann and the Dirichlet portions and defined as $\Gamma_2=L \cup \Gamma_2^N \cup \Gamma_D$.
%
%~\\
%~\\
%MY PROPOSAL FOR THIS SECTION
%~\\
%~\\
%We refer to $\isetreg_a \subset \isetreg$ as the index set of the conforming basis functions whose support has a non-null overlap with $\domain_a$, i.e.,
%$$\isetreg_a = \{ i \, : \, | \text{supp} (\mbconf{i}) \cap \domain_a | >0 \}.$$
%and to $\isetreg_L$ as the index set of the conforming basis functions whose support is non-null on the interface ${L}$, i.e.,
%$$\isetreg_L = \{ i \, : \, | \text{supp} (\mbconf{i}) \cap L | >0\}.$$
%Observe that $\isetreg_L =  \isetreg_1  \cap \isetreg_2$ and that the following partitions of unity hold
%$$\sum_{i \in \isetreg_a } \mbconf{i} (\mathbf x) =1 \quad \forall \mathbf x \in \Omega_a,$$
%for $a=\{ 1,2\}.$   
%( QUESTA FRASE NON E CHIARISSIMA, LO SPAZIO E SEMPRE LOCALE? Ho spostato la farse su in quanto uso gli spazi anche pr la conservazione globale. Non so se occorre restringere gli spazi a $\domain_a$.)
%We assume that the function spaces defined in Eq.~\eqref{eq:discretespacedefinition} are spanned by the conforming basis functions $\mbconf{i}$
%and we.

We refer to $\isetreg_L$ as the index set of the conforming basis functions whose support is non-null on the interface ${L}$, i.e.,
$$\isetreg_L = \{ i \, : \, | \text{supp} (\mbconf{i}) \cap L | >0\}.$$
and introduce the function space  $G_{L}^h =  \mathrm{span}  \{ \mbconf{i} \}_{\{i \in \isetreg_L \}}$. We also define the bilinear form and the linear functional restricted to the subdomain $\domain_a$ for $a=\{ 1,2\}$ as follows:
$$d_a({p},{q}) =  \int_{\domain_1} k \, \nabla p \cdot \nabla q \,\text{d}\Omega \quad \text{and} \quad f_a(q )=\int_{\Gamma_a^N} h \, {q} \,\text{d}\Gamma,$$
with $a=\{ 1,2\}$.

%In order to prove the local conservation property, we restrict the FE problem~\eqref{eq:flowweakdiscrete} to the subdomain $\domain_1$:
%\begin{equation}
%\label{eq:flowweak2}
%%\boxed{f
%\begin{array}{l}
%\text{Find } \hh{p}\in U^h\, \text{ such that }\\[2mm]
%d_a(  \hh{p}, \hh{v} ) = f_1(\hh{v})\quad \forall \hh{v} \in V^h.
%\end{array}
%%}
%\end{equation}

In order to derive the local conservation, we denote by $\mflux{\domain_1}{L} $ the approximated flux across the boundary $L$ with respect to $\domain_1$.

The boundary flux  $\mflux{\domain_1}{L} $ is the solution of following formulation:
\begin{equation}
\begin{array}{l}
\text{Find} \,(\hh{p},\mflux{\domain_1}{L})\in U^h\times G_{L}^h \, \text{ such that }\\[2mm]
\label{eq:bflow_local_1}
(\hh{v}, \mflux{\domain_1}{L})_{L}=d_1(\hh{p}, \hh{v}) - f_1(\hh{v})\quad\forall \hh{v}\in S^h,
\end{array}
\end{equation}
%where $\mflux{\domain_1}{L} = \sum_{J_1^r} N_A^r H(\domain_1)$ is the approximatd flux across the boundary $L$.
which can be split into two sub-problems:
\begin{align}
\nonumber
\text{Find} \,(\hh{p},\mflux{\domain_1}{L})\in U^h\times G_{L}^h \, \text{ such that }\\[2mm]
\nonumber
d_1(\hh{p}, \hh{v}) - f_1(\hh{v})&=0 & \forall \hh{v}\in \mS^h- G_{L}^h,\\
\nonumber
(\hh{v}, \mflux{\domain_1}{L})_{L} & = d_1(\hh{p}, \hh{v}) - f_1(\hh{v}) & \forall \hh{v}\in  G_{L}^h.\quad\quad
\end{align}

In the same way, one can define the flux for the complementary domain $\mflux{\domain_2}{L}$ across the boundary $L$ as the solution of the problem: 
\begin{equation}
\begin{array}{l}
\text{Find} \,(\hh{p},\mflux{\domain_2}{L})\in U^h\times G_{L}^h \, \text{ such that }\\[2mm]
\label{eq:bflow_local_2}
(\hh{v},\mflux{\domain_2}{L})_{L}=d_{2}(\hh{p}, \hh{v}) - f_{2}(\hh{v})-(\hh{v},q_D(\Omega))_{\Gamma_D} \quad \forall \hh{v}\in \mS^h,
\end{array}
\end{equation}
%\begin{align}
%\label{eq:auxflow_local_2}
%\text{Given}\, q_D(\Omega)\in G^h, \text{find} \,(\hh{p},\mflux{\domain_2}{L})\in U^h\times  G_{L}^h \, \text{ such that }\\[2mm]
%\nonumber
%d_2(\hh{p}, \hh{v}) - f_2(\hh{v})&=0 & \forall \hh{v}\in S^h-G_{L}^h,\\
%\nonumber
%(\hh{v},\mflux{\domain_2}{L})_{L}+(\hh{v},q_D(\Omega))_{\Gamma_D}-d_{2}(\hh{p}, \hh{v}) + f_{2}(\hh{v})&=0 & \forall \hh{v}\in G_{L}^h.
%\end{align}

In order to establish the local conservation, we first show that the interface fluxes, $\mflux{\domain_1}{L}$ and $\mflux{\domain_2}{L} $ are conservative with respect to corresponding subdomains $\domain_1$ and $\domain_2$. Hence, selecting any $\hh{v}\in\mS^h$ such that $\hh{v}_{\domain_a}=1$ with $a\in\{1,2\}$ leads to:
\begin{equation*}
\int_{L}\mflux{\domain_1}{L}\,\text{d}\Gamma+ \int_{\Gamma_1^N} u_N \,\text{d}\Gamma=0
\end{equation*}
and
\begin{equation*}
\int_{L}\mflux{\domain_2}{L}\,\text{d}\Gamma+ \int_{\Gamma_2^N} u_N \,\text{d}\Gamma+\int_{\Gamma_D}q_D^h(\Omega)\,\text{d}\Gamma=0.
\end{equation*}

It only remains to prove the uniqueness of the boundary flux over $L$. To this aim, we sum together Eq.~\ref{eq:bflow_local_1} and Eq. \ref{eq:bflow_local_2} and restrict $\hh{v}$ to $G_{L}^h\subset \mS^h$, thus obtaining
\begin{equation*}
(\hh{v},\mflux{\domain_1}{L}+ \mflux{\domain_2}{L})_{L}=0
\end{equation*}
%$$\mflux{\domain_1}{L}+\mflux{\domain_2}{L}=0.$$
which states that two fluxes equilibrate on $L$ and complete the proof.

{\bf Remark 1}  If the vertices of the  interface  $L$ correspond to the vertices the mesh $\mathcal{T}$, the local conservation is attained pointwise:
$$\mflux{\domain_1}{L}+\mflux{\domain_2}{L}=0.$$
and the coefficients of the boundary fluxes can be obtained by computing the inverse of a boundary mass matrix restricted to $L$.
% IF THE TWO SUBDOMAINS ARE COMPOSED OF SETS OF MESH ELEMENTS, THE INTERFACE L IS RESOLVED BY THE MESH.


{\bf Remark 2} Given the properties of the discrete diffusion operator listed in Def.~\ref{def:4}, all the results hold true also for the stabilized formulation.
%BEING THE ALGEBRAIC DIFFUSION OPERATORS SUMMING TO ZERO PER ROW AND COLUMNS, THE OBTAINED RESULTS HOLD TRUE ALSO THE STABILIZED FORMULATIONS INTRODUCED IN THE PREVIOUS SECTION. REMIND THAT THE PRROF IS BASED ON PARTITION OF UNITY/ROW SUM


\begin{itemize}
\item Non vedo dove gli spazi $J^r_1$ sono utilizzate ( In effetti non lo uso, per ora l'ho tolto)
\item Secondo me la definizione piu' corretta e' quella che ho messo sopra, perhce' e' basata sulle basis functions e non sui nodi
\item Ho visto che $\Omega_1$ e $\Omega_2$ non sono legati agli elementi della mesh, e questa cosa secondo me e giusta perche questa ipotesi non serve
\item scriverei una definizione di $d_{\Omega_a}()$ e  $F_{\Omega_a}()$ con $a$ generico cosi si fa una volta sola
\end{itemize}

%We refer to $\isetreg_1\subset \isetreg$ as the set of regular nodes lying in $\domain_1$:
%$$\isetreg_1 = \{ i \, : \, \mpoint{x}_i \in \domain_1 \},$$
%and to $\isetreg_L$ as the set of nodes residing on the boundary ${L}$:
%$$\isetreg_L = \{ i \, : \, \mpoint{x}_i \in L\}.$$
%
%We assume that the function spaces defined in Eq.~\eqref{eq:discretespacedefinition} are spanned by the conforming basis functions $\mbconf{i}$, and define $G_{L}^h$ as the span of those functions associated with the nodes of the boundary ${L}$,~i.e $G_{L}^h=\mathrm{span}\{N_a^r\}_{\isetreg_L}$. 
%We point out that the basis functions  $\mbconf{i}$ having support on $\domain_1$ are truncated and form a partition of unity,~i.e. their support, $\text{supp} N_A^r$, is locally finite and their sum gives the unity, $\sum_{\isetreg_1}N_A^r=1$. 
%
%
%In order to derive the local conservation we start with restricting the Galerkin formulation of the flow problem~\eqref{eq:flowweakdiscrete} to the subdomain $\domain_1$:
%\begin{equation}
%\label{eq:flowweak2}
%%\boxed{f
%\begin{array}{l}
%\text{Find } \hh{p}\in U^h\, \text{ such that }\\[2mm]
%d_1( \nabla \hh{p}, \hh{v} ) = f_1(\hh{v})\quad \forall \hh{v} \in V^h
%\end{array}
%%}
%\end{equation}
%where
%$$d_1(\hh{p},\hh{v}) =  \int_{\domain_1} k \, \nabla \hh{p} \cdot \nabla \hh{v} \,\text{d}\Omega \quad \text{and} \quad f_1(\hh{v})=\int_{\gamma_1^N} u_N \, \hh{v} \,\text{d}\Gamma.$$
%
%We denote by $\mflux{\domain_1}{L} = \sum_{J_1^r} N_A^r H(\domain_1)$ the approximated flux across the boundary $L$ and introduce the following Galerkin formulation:
%\begin{equation}
%\label{eq:auxflow_local_1}
%%\boxed{
%\begin{array}{l}
%\text{Find} \,(\hh{p},\mflux{\domain_1}{L})\in U^h\times G_{L}^h \, \text{ such that }\\[2mm]
%d_1(\hh{p}, \hh{v}) - f_1(\hh{v})=(\hh{v}, \mflux{\domain_1}{L})_{L}\,\,\forall \hh{v}\in S^h,
%\end{array}
%\end{equation}
%%where $\mflux{\domain_1}{L} = \sum_{J_1^r} N_A^r H(\domain_1)$ is the approximatd flux across the boundary $L$.
%which can be split into two sub-problems:
%\begin{align}
%\nonumber
%\text{Find} \,(\hh{p},\mflux{\domain_1}{L})\in U^h\times G_{L}^h \, \text{ such that }\\[2mm]
%\nonumber
%0=&d_1(\hh{p}, \hh{v}) - f_1(\hh{v})\,\,\,\forall \hh{v}\in S^h- G_{L}^h,\\
%\nonumber
%(\hh{v}, \mflux{\domain_1}{L})_{L}=&d_1(\hh{p}, \hh{v}) - f_1(\hh{v})\,\,\,\forall \hh{v}\in  G_{L}^h.\quad\quad
%\end{align}
%As already pointed out for the evaluation of the Dirichlet flux $\mflux{\domain}{D}$, the \textit{post-processing} computation of the boundary flux $\mflux{\domain_1}{L}$ requires the inversion of a boundary mass matrix.
%
%In the same way, one can define the flux for the complementary domain $\mflux{\domain_2}{L}$ across the boundary $L$ as the solution of the problem: 
%\begin{align}
%\label{eq:auxflow_local_2}
%\text{Given}\, q_D(\Omega)\in G^h, \text{find} \,(\hh{p},\mflux{\domain_2}{L})\in U^h\times  G_{L}^h \, \text{ such that }\\[2mm]
%\nonumber
%0=d_2(\hh{p}, \hh{v}) - f_2(\hh{v})&\,\,\forall \hh{v}\in S^h-G_{L}^h,\\
%\nonumber
%(\hh{v},\mflux{\domain_2}{L})_{L}=d_{2}(\hh{p}, \hh{v}) - f_{2}(\hh{v})-(\hh{v},q_D(\Omega))_{\Gamma_D}&\,\,\forall \hh{v}\in  G_{L}^h\quad\quad\quad
%\end{align}
%where  
%$$d_{2}(\hh{p},\hh{v}) =  \int_{\domain_2}\, \nabla \hh{p} \cdot \nabla \hh{v} \,\text{d}\Omega \quad \text{and} \quad f_{2}(\hh{v})=\int_{\Gamma_2^N} u_N \, \hh{v} \,\text{d}\Gamma.$$
%
%We establish the local conservation by proving that subdomain interface fluxes, $\mflux{\domain_1}{L}$ and $\mflux{\domain_2}{L} $  equilibrate pointwise and are conservative with respect to the subdomains $\domain_1$ and $\domain_2$, respectively. Indeed,  selecting $\hh{v}|_{\domain_j}=1$ with $j\in\{1,2\}$ leads to:
%$$\int_{L}\mflux{\domain_1}{L}\,\text{d}\Gamma+ \int_{\gamma_1^N} u_N \,\text{d}\Gamma=0$$
%and
%$$\int_{L}\mflux{\domain_2}{L}\,\text{d}\Gamma+ \int_{\Gamma_2^N} u_N \,\text{d}\Gamma+\int_{\Gamma_D}q_D^h(\Omega)\,\text{d}\Gamma=0.$$
%Hence, summing together Eq.~\eqref{eq:auxflow_local_1} and Eq. \eqref{eq:auxflow_local_2} and restricting $\hh{v}$ to $G_{L}^h\subset S^h$ allows to attain the local conservation property for the continuous Galerkin method, ~i.e:
%$$\mflux{\domain_1}{L}+\mflux{\domain_2}{L}=0$$
%
%\textbf{Remark}
%We point out that the same property can be established for any arbitrary catting curve   $L=\domain_1\cap\domain_2$ whose vertices do not necessarily correspond to the vertices the mesh $\mathcal{T}$.

==> sections/05Results.tex <==
\section{Numerical examples}

In this section, we show the conservation properties and positivity of the solution for FE discretization on adapted meshes with hanging nodes.



simulation of equi-dimensional models for coupled flow and transport in fractured porous media with FE method.
For the flow problem, we focus both on the conservation properties of the computed fluxes and on the positivity of the solution.
For the transport problem, the main focus is to show the positivity of the concentrations.

We show for porous fractured

the numerical methods presented in Section 3. First, in Section 4.1, we consider a pure transport problem where the velocity is given explicitly and the exact solution is known. This is to verify our transport model, Eq. (3.29), and in particular our approximation of the coupling term, see Eq. (3.16).
Next, in Section 4.2, we consider two benchmark cases for the pure pressure problem presented in [32]. The first case is a regular fracture network, while the second problem is a realistic case with a complex fracture network. The aim is to compare EFEM, Eq. (3.10), to other DFM models for single-phase flow.


Finally, in Section 4.3, we solve the coupled pressure and transport problem in the same cases as in Section 4.2. This will reveal the capabilities of our solution approach.
All computer implementation of the numerical methods are based on the open-source software deal.II [42] and are freely available under an open license.1 We only consider 2D problems, but our fracture model and numerical methods can be applied to 3D problems as well. All meshes are built up of quadrilateral elements. The meshes may be locally refined by recursively dividing selected elements in four, but we allow for no more than one hanging node per element face. The number of degrees of freedom is denoted Ndof.



In this section, we validate the proposed approach using five benchmark cases. The first benchmark is s a two-dimensional version of the test case proposed in~\cite{BenchPaper}
The second benchmark case is based on Geiger et al. (2013) ~\cite{flemisch2018benchmarks} and shows a regular fracture network. The third test case is based on a well-established benchmark for groundwater flow from Swedish Nuclear Power Inspectorate (SKI) (1987). The fourth taste case is a three-dimensional test case containing small geometric features~\cite{BenchPaper}, whereas the last benchmark considers a realistic scenario where several fractures randomly oriented are embedded in a rock matrix.

For each benchmark,  we consider both the resolved and the unresolved test cases and compare the numerical results in terms of pressure and concentration profiles along the prescribed lines.


\subsection{Adaptive mesh refinement\\ for heterogenous media}

In this section, we briefly summarize the AMR method, whose details are presented in \cite{Holliger2000}.
The idea at the base is to start with a coarse uniform mesh.
In particular, for cuboid domains of tipe $\Omega^c$,
the initial mesh can also be thought as structured.
The initial mesh is not supposed to explicitly resolved the interfaces between the background and the fractures.

Then, given a distribution of embedded fractures,
we iterate over all elements and mark for refinement the ones that have non-empty intersections with the boundary of at least one fracture.

In some cases, it can be useful to change the target according to which we decide to mark for refinement.
For example, when conductive fractures are considered, i.e., fractures which have a permeability much larger compared to the one of the matrix,
it is convenient to mark for refinement all the elements that have a non-empty overlap with at least one fracture.
This means that elements insides a fracture are refined as well.
Moreover, the refinement region can be a region around the fracture but not necessarily coinciding with the fracture.


This procedure allows to create a sequence of meshes, which become progressively finer towards the interfaces.
This AMR method allows to automatically create meshes for any heterogeneity distribution without any human interaction.
In order to keep the meshes $1$-irregular, at each step the refinement region may be enlarged in order to satisfy such a constraint.


%In order to evaluate the accuracy of the method, solutions or output variables, such as seismic attenuation and velocity dispersion,
%from two consecutive hierarchical levels can be compared.

%Another possibility for evaluating the quality of the solution would be to employ error estimators,
%which are not readily available for the proposed method.
%In this regard, there are basically two options.
%One would be to adapt error estimators based on flux reconstruction that have already been developed for Biot's equations in the time domain \cite{RIEDLBECK20171593}.
%Here, the main difficulty would be to extend this methodology to complex vector spaces and non-symmetric problems.
%Another would be to use more generic residual-based error estimators for coupled problems, e.g. \cite{ern2009posteriori}.


\subsection*{Resolved and unresolved discretizations}
We finally introduce two different methods to simulate flow and transport in fractured media.

\textit{Resolved discretization} The first discretization will be referred to as \emph{resolved} and its meshes resolve the interfaces between the matrix and the fractures. It makes use of conforming meshes which are, in general, complicated to generate,
since they require a lot of human-computer interaction to achieve the desired mesh quality. The mesh generation of a fractured network system is usually tedious and difficult  to make automatic due to the geometric complexity of the computational domain induced by existence and extension of fractures.

\textit{Unresolved discretization} The second discretization will be referred to as \emph{unresolved} and its meshes do not explicitly resolve the interfaces between the matrix and the fractures,
but are actually refined close to such interfaces. More specifically an adaptive refinement procedure is adopted to ensure the desired leyer of elements inside  each fracture network. Given a mesh $\mathcal{T}$, each element is initially marked as belonging to either the background matrix or to the fracture network. Then all the elements marked as \textit{fractured} are progressively refined until the desired mesh-accuracy is achieved.

\textbf{Remark} For the unresolved discretization, all the bilinear and linear operators, i.e matrices and vectors, are computed element-wise on the non-conforming space $W^H$ and them projected onto the regular space $V^r$ by means of the interpolation operator~\eqref{eq:interp}.

It is worth to pointing out that, the stabilization of the transport problem can be also either performed on the  transport operator $\mathbf{A}$ or on its element-wise contribution $[\mathbf{A}]_{ij}$ . While there is no difference between the two approaches when conforming meshes are adopted, the use of non-conforming meshes makes mandatory the first approach. Indeed, if one stabilize the local contribution $[\mathbf{A}]_{ij}$, the subsequent use of the relation $\eqref{eq:intA}$ introduces off diagonal entries which violate the assumptions 1a and 1b of theorem~\ref{th:DM} needed to ensure the DMP.

According to the definitions above, a triangulation can be non-conforming and non-uniform but all elements are shape-regular, being squares or cubes.



%\textbf{It is also a very tedious task to create a full-dimensional description of the fracture network and a corresponding equi-dimensional grid of the whole computational domain. Therefore, we refrain from calculating a reference solution with the MFD method and per- form a direct comparison of the hybrid-dimensional methods.
%It is also a very tedious task to create a full-dimensional description of the fracture network and a corresponding equi-dimen- sional grid of the whole computational domain. Therefore, we refrain from calculating a reference solution with the MFD method and per- form a direct comparison of the hybrid-dimensional methods..}

%Ciò che inficia la regolarità sono i jump nei parametri (mi sembra che la sol appartenga a H^5/4) e particolari cambi di boundary conditions (La sol è meno di H^2). A priori entrambi questi problemi riducono la convergenza dei metodi fe, in quanto la sol deve essere almeno in p+1 al fine di avere convergenza con ordine p. Il converence rate ridotto dovuto ai jump nei parametri può essere evitato con mesh che risolvono i boundary delle discontinuità. In questo caso si ottengono ordini di convergenza simili al problema senza discontinuità, con il fatto che se ci sono molte discontinuità sono difficili da meshare. Invece il problema legato alla discontinuità del tipo di boundary conditions non può essere evitato in alcun modo con i fe standard. Possibili soluzioni sono usare metodi GFEM o multiscala che aggiungono particolari funzioni legate al tipo di discontinuità oppure provare a fare AMR vicino al cambio del tipo di boundary conditions.}


\subsection{Single 2D}
%\begin{enumerate}
%\item good agreement between unresolved and resolved
%\item for the resolved case meshes comprising poor-quality elements may affect the accuracy of the method as shown in Figure~2
%\end{enumerate}
The first benchmark example consists of a square-shaped domain $\Omega_{M}$ crossed by a an oblique fracture $\Omega_{F}$ with a thickness $\delta=0.01$. To represent an heterogeneous rock matrix, different material properties are assigned to a sub-domain $\Omega_{het}$ defined in lower part of the domain $M$.  A geometrical description of the rock matrix and the fracture are depicted in Figure, whereas more details on the geometrical sizes can be found in Table~\ref{tab:geo_1}.
\begin{table}[ht]
\caption{Geometrical sizes}
\centering
\begin{tabular}{ |p{1cm}||p{1cm}|p{1cm}|p{1cm}| |p{1cm}|  }
 \hline
 \multicolumn{5}{|c|}{Rock Matrix} \\
 \hline
      & {$\bf{x_{s}}$} [m]& $\bf{x_{e}}$ [m]& $\bf y_{s}$ [m]& $\bf y_{e}$ [m] \\
 \hline
$\mathrm\Omega_{M}$ &-50 & 50 & -50 & 50    \\
$\mathrm\Omega_{het}$  &-50 & 50 & -50 & -40  \\
$\mathrm{\Gamma_{in}}$  &0 & 0 & 40 & 50  \\
$\mathrm{\Gamma_{out}}$  &50 & 50 & 0 & 10  \\
 \hline
 \multicolumn{5}{|c|}{Fracture} \\
  \hline
      & $ \bf x_{s}$ [m]& $\bf x_{e}$ [m]& $\bf y_{s}$ [m]& $\bf y_{e}$ [m]  \\
 \hline
 $\mathrm\Omega_{F}$& -50   & 50 & -30 & 30\\
 \hline
\end{tabular}
\label{tab:geo_1}
\end{table}

Concerning the boundary conditions, for the flow problem, we impose a Dirichlet condition at the inlet $\Gamma_in$ with $p_{in}^{D}= 4m$ and at the outlet $\Gamma_{out}$ with $p_{out}^{D} = 1m$,  whereas for the transport problem, we impose a Dirichlet condition $c_{in}^{D} = 0.01m^{2}$ at the inlet $\Gamma_{in}$.  For the transport problem, the overall simulation time is $t_f=10^{9}\,\rm{[s]}$ and the time step is $dt=10^2~\rm{[s]}$. The parameters adopted for the material properties are summarized in Table~\ref{tab:geo_1}. 


\begin{table}[ht]
\caption{Parameters Setting for conductivity and porosity}
\centering
\begin{tabular}{ |p{4cm}||p{1cm}|}
 \hline
 \multicolumn{2}{|c|}{Parameters Values} \\
 \hline
matrix conductivity $\bf K_{M1}$    &  $10^{-6}$ \\
matrix conductivity $\bf K_{M2}$    &  $10^{-5}$ \\
fracture conductivity $\bf K_{F}$     &   $10^{-1}$ \\
matrix porosity$\boldsymbol{\phi_{M1}}$    & $0.2 $ \\
matrix porosity $\boldsymbol{\phi_{M2}}$   & $0.2$  \\
matrix porosity $\boldsymbol{\phi_{M3}}$   &  $0.25$ \\
fracture porosity$\boldsymbol{\phi_{F}}$      & $0.4$\\
 \hline
\end{tabular}
\label{tab:param_1}
\end{table}

Four different meshes are considered for the resolved and the unresolved configurations. In Table~\ref{tab:mesh_1} we report the number of nodes, elements and layer of elements inside the fracture for each test case. 
\begin{figure}[hbt!]
\centering
\includegraphics[width=9cm]{figures_new/single/fig_mesh_unres}
\caption{Locally refined mesh for the test case $\rm{unres_3}$. }
\label{fig:single_unresolved_mesh}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm ]{figures_new/single_p}
\caption{Pressure distribution for the test case $\rm{unres_3}$ (Units [Pa]).}
\label{fig:single_p_unresolved_setup}
\end{figure}

%\begin{figure}[hbt!]
%\centering
%\hspace{0.1cm}
%\includegraphics[width=11cm ]{figures_new/single/single_c_tot}
%\caption{Concentration distribution at time $t=2\,10^{8}[s]$ and $t=\,10^{9}[s]$ for the test case $\rm{unres_3}$ (Units [m]).}
%\label{fig:unresolved_single_c}
%\end{figure}

As an example, in Figures~\ref{fig:single_unresolved_mesh}, \ref{fig:single_p_unresolved_setup} and~\ref{fig:unresolved_single_c} we show  the mesh used for the test case $\mathrm{unres_3}$,   the corresponding solution obtained by solving the flow problem, and  the one resulting from the transport problem, respectively. In particular, we in Figure~\ref{fig:unresolved_single_c} we show the concentration distribution at the time instants $t=2\,10^{8}[s]$ and $t=\,10^{9}[s]$.  The obtained results confirm the ability of  stabilization technique to preserve the positivity of the solution and ensure the local maximum principle.


\begin{table}[ht]
\caption{Mesh Setting for Benchmark Single 2D}
\centering
\begin{tabular}{ |p{2cm}|p{2cm}|p{2cm}|p{1cm}|p{2cm}|p{2cm}|  }
 \hline
 \multicolumn{6}{|c|}{Resolved Mesh} \\
 \hline
      &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
$\mathrm{res_1}$&\,\,\,\,\,\,\,6\,785  &\,\,\,\,\,\,\,6\,612 &  1& $1.86675\,e^{-6}$  & $-1.86675\,e^{-6}$\\
$\mathrm{res_2}$&\,\,\,26\,793  &\,\,\,\,26\,448 &  2& $1.85977\,e^{-6}$  & $-1.85977\,e^{-6}$\\
$\mathrm{res_3}$& 106\,481  & 105\,792 &  3& $1.85632\,e^{-6}$  & $-1.85632\,e^{-6}$\\
$\mathrm{res_4}$& 424\,545  & 423\,168 &  4& $1.85457\,e^{-6}$  & $-1.85457\,e^{-6}$\\
 \hline
 \multicolumn{6}{|c|}{Unresolved Mesh} \\
  \hline
        &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
 $\mathrm{unres_1}$&\,\,\,\,162\,628   &\,\,\,\,141\,640  & 1.28  & $1.86277\,e^{-6}$ & $-1.86277\,e^{-6}$\\
  $\mathrm{unres_2}$&\,\,\,\,401\,680   &\,\,\,\,442\,813  & 2.56  & $1.85779\,e^{-6}$ & $-1.85779\,e^{-6}$\\
 $\mathrm{unres _3}$&1\,291\,360      &1\,375\,252 & 5.12       &$1.85534\,e^{-6}$ & $-1.85534\,e^{-6}$ \\
 $\mathrm{unres _4}$&2\,678\,304      &2\,512\,480 &10.24      & $1.85517\,e^{-6}$ & $-1.85517\,e^{-6}$ \\
 \hline
\end{tabular}
\label{tab:mesh_1}
\end{table}




\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/single/conservation}
\caption{Flux conservation}
\label{fig:single_flux}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/single/pressure}
\caption{Pressure Profile}
\label{fig:single_P}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/single/concentration}
\caption{Concentration}
\label{fig:single_CM}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=8cm]{figures_new/single/fig_mesh_res}
\caption{Left: mesh of the test case $\rm{res_{1,\rm{uni}}}$ together with a zoom-in of the region close to end point $\rm B^{\prime}$. Right: comparison between  the concentration profiled obtained for the test cases $\rm{res_{1,\rm{uni}}}$  and  $\rm{res_1}$ along the line $\rm{B-B^{\prime}}$.}
\label{fig:mesh_c_recolved_bench_1}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/single/concentration_correction_2}
\caption{Concentration distribution at time $t=2\,10^{8}[s]$ and $t=\,10^{9}[s]$ for the test case $\rm{unres_3}$ (Units [m]).}
\label{fig:unresolved_single_c}
\end{figure}

%\begin{figure}[hbt!]
%\includegraphics[width=6cm]{figures_new/single/resolved/fig_1}
%\includegraphics[width=6cm]{figures_new/single/unresolved/fig_1}
%\caption{Pressure profiles along the line $\rm{A-A^{\prime}}$ for all the resolved (left) and unresolved (right) cases presented in Table~\ref{tab:mesh_1}. }
%\label{fig:figure_p_res_unres_bench1}
%\end{figure}
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=7cm]{figures_new/single/fig_1}
%\caption{Pressure profiles along the line $\rm{A-A^{\prime}}$ for the finest resolved and unresolved test cases, respectively.}
%\label{fig:figure_p_comp_bench1}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/single/resolved/fig_2}
%\includegraphics[width=6cm]{figures_new/single/unresolved/fig_2}
%\caption{Concentration profiles  at final time along the line $\rm{A-A^{\prime}}$ for all the resolved (left) and unresolved (right) cases presented in Table~\ref{tab:mesh_1}. }
%\label{fig:figure_c1_bench1}
%\end{figure}


%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/single/resolved/fig_3}
%\includegraphics[width=6cm]{figures_new/single/unresolved/fig_3}
%\caption{Concentration profiles  at final time along the line $\rm{B-B^{\prime}}$ for all the resolved (left) and unresolved (right) cases presented in Table~\ref{tab:mesh_1}.}
%\label{fig:figure_c2_bench1}
%\end{figure}
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/single/fig_3}
%\includegraphics[width=6cm]{figures_new/single/fig_2}
%\caption{Concentration profiles  at time $t=t_f$ along the line $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for the finest resolved and the unresolved test case, respectively.}
%\label{fig:figure_c_comp_bench1}
%\end{figure}







We validate our approach by analyzing the pressure and the concentration profiles along the lines connecting the points $\rm{A-A^{\prime}}$, with coordinates $\rm{A}=(50;-50;0)$, and $\rm{A^{\prime}}=(-50;50;0))$, and $\rm{B-B^{\prime}}$, with coordinates $\rm{B}=(30;-30;0)$, and $\rm{B^{\prime}}=(-30;30;0))$, as depicted in Figure~\ref{fig:single_p_unresolved_setup}.

In Figures~\ref{fig:figure_p_res_unres_bench1} and~\ref{fig:figure_p_comp_bench1} we compare the pressure computed along the line $\rm{A-A^{\prime}}$ for all the test cases presented in Table~\ref{tab:mesh_1}. No relevant differences are found among all the numerical results (Figure~\ref{fig:figure_p_res_unres_bench1}) and a good agreement is observed between the resolved and the unresolved solution (Figure~\ref{fig:figure_p_comp_bench1}).


In Figures~\ref{fig:figure_c1_bench1} and ~\ref{fig:figure_c2_bench1} the concentration obtained at time $t=t_f$ along the lines $\rm{A-A^{\prime}}$ and  $\rm{B-B^{\prime}}$ is plotted. Again, all the analyzed profiles reveal a similar behaviour and a good match is found between the resolved and the unresolved results, as shown in Figure~\ref{fig:figure_c_comp_bench1}.

It is worth pointing out that the use of adaptive refinement allows controlling the quality of the mesh which represents an important requirement to ensure the stability of the method and accuracy of the solution. In this regard, in Figure~\ref{fig:mesh_c_recolved_bench_1} we show a comparison between the concentration obtained for the test cases $\rm{res_{1,\rm{uni}}}$ and $\rm{res_1}$ along the line $\rm{B-B^{\prime}}$. Differences can be clearly observed close to the endpoint $\rm{B^{\prime}}$ and are mainly related to the poor-quality of the mesh $\rm{res_{1,\rm{uni}}}$ obtained by performing one uniform refinement step on the mesh used for the test case $\rm{res_{1}}$.




\subsection{Regular}
%\begin{enumerate}
%\item good agreement between unresolved and resolved
%\item for the unresolved we observe a deviation the solution along line 2 whereas along line 1 (fracture in the middle) we get good match for both the resolved the unresolved meshes.
%Can we justify the deviation with the low order of convergence due to the discontinuity in both parameters and boundary conditions? this hypothesis seems to be supported from the fact that in the blocking case we get good agreement with respect to the reference solution for both resolved and the unresolved mesh. 
%\item for the concentration can we justify the differences between the resolved and the unresolved case in the same way as done for the pressure?
%\item for the plots over region the concentration seems to tend to zero in regions 2 4 and 6 (figure 18). The diffusion added by the stabilization term seems to prevent the solution to go to zero (shell we mention this?). Can  we refer to the  differences between the solutions in these regions to justify also the differences obtained in the plots over line (see figures~15 and 17)?
%\end{enumerate}

The second benchmark consists of a regular fracture network embedded in square with size $x_s=0\,m\,x_e=1\,m$ and $y_s=0\,m\,y_e=1\,m$. The rock has a unitary conductivity $K_M = I$, whereas for the fractures we consider two cases: a highly conductive fracture network with $K_F = 10^4$ and a blocking fracture network with $K_F=10^{-4}$. For the transport problem, the matrix and the fracture network have the same porosity,~i.e. $\phi_m=\phi_f=1.0$.

For the flow problem, we apply homogeneous Neumann conditions (no flow) on top and bottom sides, a unitary inflow flux $u_N=-1$ on the left boundary, and a Dirichlet condition $p_D = 1$ on the right boundary. Our numerical results are compared with the numerical approaches and the reference solution presented in~\cite{flemisch2018benchmarks}. 

For the transport problem, a unitary concentration $c_d=1.0$ is imposed on the left boundary, whereas homogeneous Neumann conditions (no flow) are applied on the remaining sides.  The time step $dt=0.025~\rm{[s]}$ and the overall simulation time is set equal to$t_f=0.5,~\rm{[s]}$. 





%    \begin{figure}[hbt!]
%    \centering
%    \includegraphics[width=3.8cm]{figures/regular/RegularConfC1.eps}
%    \includegraphics[width=3.8cm]{figures/regular/RegularAMRC1.eps}
%    \includegraphics[width=3.8cm]{figures/regular/RegularConfAMRC1.eps}
%    \caption{Benchmark 2 with conductive fractures: comparison of concentration values along the line $y=0.5$}
%    \label{fig:figure_p1_bench2}
%    \end{figure}

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=3.8cm]{figures/regular/REgularConfC2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularAMRC2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularConfAMRC2.eps}
%\caption{Benchmark 2 with conductive fractures: comparison of concentration values along the line $y=0.5$}
%\label{fig:figure_p1_bench2}
%\end{figure}

% \begin{figure}[hbt!]
% \centering
% \includegraphics[width=8cm]{figures/RegularVerticalLine}
% \caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $x=0.5$.}
% \label{fig:figure_p2_bench2}
% \end{figure}




\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm]{figures_new/regular_p}
\caption{Pressure distribution for the test case $\rm{unres_3}$ (Units [Pa])}
\label{fig:unresolved_regular_p}
\end{figure}


%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=10cm]{figures_new/regular_c_tot}
%\caption{Concentration distribution at time $t=\,0.20[s]$ and $t=\,0.5[s]$ for the test case $\rm{unres_3}$ (Units [m]).}
%\label{fig:unresolved_regular_c}
%\end{figure}

\subsubsection{Conductive fracture network}
First, we consider a highly conductivity network. Three different meshes are considered for the resolved and the unresolved configurations. In Table ~\ref{tab:mesh_2} we report the number of nodes, elements and layer of elements inside the fracture for each test case.

\begin{table}[ht]
\caption{Mesh Setting for Benchmark Regular 2D}
\centering
\begin{tabular}{ |p{2cm}|p{2cm}|p{2cm}|p{1cm}|p{2cm}|p{2cm}|  }
 \hline
 \multicolumn{6}{|c|}{Resolved Mesh} \\
 \hline
      &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
%$\mathrm{unres_0}$&     29929 &   29584    &  4\\
$\mathrm{unres_1}$&   110889 &  110224    &  4&  0.662191 & -0.662191\\
$\mathrm{unres_2}$&   426409 &  425104   &  4 & 0.662189 & -0.662189\\
$\mathrm{unres_3}$&   1671849    & 1669264   &  4 & 0.662185&-0.662185\\
$\mathrm{unres_4}$&    16056049   &   16048036  &  2&  0.662177 & -0.662177\\
 \hline
 \multicolumn{6}{|c|}{Unresolved Mesh} \\
  \hline
      &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
$\mathrm{unres_1}$&  1\,863\,685 &    1\,720\,768    &  4& 0.65692& -0.65692\\
$\mathrm{unres_2}$&     1\,879\,729 &   1\,736\,896  &  4 &0.656915 &-0.656915 \\
$\mathrm{unres_3}$&    4\,673\,031     &  4\,387\,096   &  8 &0.662382 &-0.662382\\
$\mathrm{unres_4}$&      4\,966\,635   &  4\,681\,144   &  8& 0.662381& -0.662381\\
$\mathrm{unres_5}$&        15\,054\,349   &    14\,483\,152   &  16&0.662415&-0.662415\\
 \hline
\end{tabular}
\label{tab:mesh_2}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c| c |}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11\\
80 &  &  &  &  &  &  0.12045&  0.11707&  0.11704&  0.11823&  0.1182 \\
160 &  &  &  &  &  0.12031&  0.11692&  0.11691&  0.11811&  0.11808&   \\
320 &  &  &  &  0.12023&  0.11684&  0.11683&  0.11803&  0.11801&  &   \\
640 &  &  &  0.1202&  0.11679&  0.11679&  0.11799&  0.11797&  &  &   \\
1280 &  &  0.12018&  0.11677&  0.11677&  0.11797&  0.11794&  &  &  &   \\
2560 &  0.12017&  0.11676&  0.11676&  0.11796&  0.11793&  &  &  &  &   \\
\end{tabular}
\caption{flussi unresolved stab}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c| c |}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 \\
80 &  &  &  &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11776 \\
160 &  &  &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&   \\
320 &  &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &   \\
640 &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &  &   \\
1280 &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &  &  &   \\
2560 &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &  &  &  &   \\
\end{tabular}
\caption{flussi unresolved non-stab}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c| c |}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 \\
80 &  &  &  &  &  &  474.29&  951.49&  3537.8&  9321.43&  30687.04 \\
160 &  &  &  &  &  533.79&  997.24&  3541.53&  9293.61&  29055.21&   \\
320 &  &  &  &  825.26&  1305.83&  3817.38&  9345.93&  28419.23&  &   \\
640 &  &  &  1573.17&  2161.3&  4909.56&  10994.99&  29168.34&  &  &   \\
1280 &  &  5397.39&  6343.81&  9328.68&  15453.4&  37212.82&  &  &  &   \\
2560 &  10726.8&  11474.12&  13512.52&  17933.18&  31340.79&  &  &  &  &   \\
\end{tabular}
\caption{solution time non stab, decidi se torna utile}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | }
 & 1 & 2 & 4 & 8 & 16 \\
80 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11775 \\
160 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11775 \\
320 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11775 \\
640 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11776 \\
1280 &  0.11775&  0.11775&  0.11776&  0.11776&  0.11776 \\
\end{tabular}
\caption{flussi resolved}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | }
 & 1 & 2 & 4 & 8 & 16 \\
80 &  44.03&  43.74&  44.56&  33.11&  42.12 \\
160 &  59.9&  67.31&  70.1&  76.72&  96.27 \\
320 &  216.14&  212.6&  220.18&  220.88&  259.91 \\
640 &  844.39&  816.7&  918.61&  888.23&  1007.48 \\
1280 &  3678.56&  3725.55&  3476.15&  3829.14&  3680.57 \\
\end{tabular}
\caption{solution time resolved, direi che non \'e utile}
\end{table}

In Figure~\ref{fig:unresolved_regular_p} we show the spatial distribution of the pressure, and  the extreme points of the lines $A-A^{\prime}$, $(x=0.5)$, and $B-B^{\prime}$, $(y=0.75)$ along which we perform our analysis.
Figures~\ref{fig:regular_p1_res_unres} and ~\ref{fig:regular_p1_res_unres} depict the pressure profile along the line $A-A^{\prime}$ and  $B-B^{\prime}$,  for the resolved and the unresolved test cases reported in Table~\ref{tab:mesh_2}. Here, one may observe that all the solutions exhibit a similar behaviour. Figure~\ref{fig:regular_p1_p2_comp} shows a comparison with the numerical methods and the reference solution presented in ~\cite{flemisch2018benchmarks}. It refers to a very fine reference mesh, with a total of $1\,175\,056$ element, where the fractures are resolved by ten elements in their normal direction.

While all the results reveal a good match for line $A-A^{\prime}$, a small deviation is found for the test case $\rm{unres_3}$ along the line $B-B^{\prime}$, where our method shows a good agreement with the Embedded Discrete Fracture Method (EDFM).
\begin{table}[ht]
\caption{List of Regions}
\centering
\begin{tabular}{ |p{2cm}||p{2cm}|p{2cm}|  }
 \hline
      & $\mathbf{x}_{range}$    & $\mathbf{y}_{range}$ \\
       \hline
$\mathrm{1}$&  [0\,\,0.5] &   [0\,\,0.5]   \\
$\mathrm{2}$&   [0.5\,\,1.0] &   [0\,\,0.5]   \\
$\mathrm{3}$&  [0\,\,0.5]     &  [0.5\,\,1.0]    \\
$\mathrm{4}$&  [0.75\,\,1.0]     &  [0.75\,\,1.0]    \\
$\mathrm{5}$&  [0.75\,\,1.0]     &  [0.5\,\,0.75]    \\
$\mathrm{6}$&  [0.5\,\,0.75]     &  [0.75\,\,1.0]    \\
$\mathrm{7}$&  [0.5\,\,0.625]     &  [0.5\,\,0.6250]    \\
$\mathrm{8}$&  [0.625\,\,0.75]     &  [0.5\,\,0.6250]    \\
$\mathrm{9}$&  [0.5\,\,0.6255]     &  [0.625\,\,0.6250]    \\
$\mathrm{10}$&  [0.625\,\,0.75]     &  [0.625\,\,0.750]    \\
 \hline
\end{tabular}
\label{tab:regions}
\end{table}
In Figures~\ref{fig:c1_regular_res_unres} and~\ref{fig:c2_regular_res_unres}, we compare the concentration at the final time $t=t_f$ along the lines $\rm{B-B^{\prime}}$ and $\rm{C-C^{\prime}}$($y=0.5$ in Figure~\ref{fig:unresolved_regular_p}),respectively. We can observe mesh convergence for both the resolved and the unresolved test cases. In particular, while a good agreement is found among all the results related to the unresolved configuration, we observe that the difference among the solutions computed for the resolved test cases progressively reduces with mesh refinement. 
A comparison between the resolved and the unresolved test cases is performed by analyzing both the concentration along lines $B-B^{\prime}$ and $C-C^{\prime}$ and the average concentration in the regions listed in Table~\ref{tab:regions}. The two configurations reveal a good agreement for all the regions except for region $2$ where the solution obtained for the unresolved case $\rm{unres_3}$ is almost half the one computed for the resolved one $\rm{res_3}$. However, we have observed that the concentration in this region progressively decreases by uniformly refining the grid (not shown). Thus, we believe that the differences between the numerical solutions are mainly related to the artificial diffusion introduced by the stabilization which prevents the concentration to become zero.

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_res_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_unres_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_tot}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}


\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_u_r}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/cm_res_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/cm_ures_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/regular/cm_res_vs_ures_1}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/regular/cm_res_vs_ures_2}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/regular/cm_res_vs_ures_3}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures/fig_single_4}
%\includegraphics[width=8cm]{figures/fig_mesh_2}
%\caption{Concentration profiles for the benchmark \textit{single2d}  at final time along the fracture $(50\,;\,-30\,;\,0), (-50\,;\,30\,;\,0)\,m$ for the test case 4.}
%\label{fig:figure_c3_bench1}
%\end{figure}

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_3.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_4.eps}
%\caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the lines $x=0.5$ and $y=0.7$ for different conformed-mesh size}
%\label{fig:regular_p1_unres}
%\end{figure}

\clearpage

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_1.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_1.eps}
%\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
%\label{fig:regular_p1_res_unres}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_2.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_2.eps}
%\caption{Pressure along the line $B-B^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases. (Conductive)}
%\label{fig:regular_p1_res_unres}
%\end{figure}
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/fig_1}
%\includegraphics[width=6cm]{figures_new/regular/fig_2}
%\caption{Comparison among the pressure profiles along the lines $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for test cases $res_3$, $unres_3$, and the reference solution (Conductive).}
%\label{fig:regular_p1_p2_comp}
%\end{figure}

\clearpage

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=3.8cm]{figures/regular/RegularConfP1.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularAMRp1.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularVerticalLine}
%\caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $x=0.5$ for different conformed-mesh size}
%\label{fig:figure_conf_bench2}
%\end{figure}

% \begin{figure}[hbt!]
% \centering
% \includegraphics[width=8cm]{figures/RegularAmr}
% \caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $x=0.5$ for different AMR-mesh size}
% \label{fig:figure_amr_bench2}
% \end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=3.8cm]{figures/regular/RegularConfp2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularAMRp2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularHorizontalLine.png}
%\caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $y=0.7$}
%\label{fig:figure_p1_bench2}
%\end{figure}


%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_3.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_5.eps}
%\caption{Concentration at final time $t=0.5~[s]$ along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
%\label{fig:c1_regular_res_unres}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_4.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_6.eps}
%\caption{Comparison among the concentration profiles along the lines $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for test cases $res_3$, $unres_3$ (Conductive).}
%\label{fig:c1_c2_regular_res_unres}
%\end{figure}
%
%
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/fig_3}
%\includegraphics[width=6cm]{figures_new/regular/fig_4}
%\caption{Concentration at final time $t=0.5~[s]$ along the line $B-B^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
%\label{fig:c2_regular_res_unres}
%\end{figure}
%
%
%
%
%\begin{figure}[hbt!]
%\hspace{-0.8cm}\includegraphics[width=12cm]{figures_new/regular/fig_5}
%\caption{Average concentration in the regions defined in~\ref{tab:regions} over time (Conductive).}
%\label{fig:figure_c_bench2}
%\end{figure}
%
%
%\subsubsection{Blocking fracture network}
%We now present the numerical results obtained for the blocking fracture network. In particular, we focus on the comparison between the numerical results obtained by solving the flow problem on the resolved and the unresolved meshed reported in Table~\ref{tab:mesh_2}. As an example, the pressure distribution is shown in Figure~\ref{fig:regular_blocking_p} where 
%one may observe the pressure discontinuities induced by the low fracture permeability.
%Figures~\ref{fig:regular_res_unres_p_blocking} and ~\ref{fig:comparison_res_unres_p_blocking} depict the pressure profile along the line $\rm{A-A^{\prime}}$, with coordinated $A=(0.1,0,0)$ and $A^{\prime}=(1.0,0.9,0)$ . Again a good agreement is found among all the numerical solutions.
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=7cm]{figures_new/regular_p_blocking_2}
%\caption{Pressure distribution for unresolved test case $\rm{unres_3}$ (Blocking).}
%\label{fig:regular_blocking_p}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular_blocking/resolved/fig_1}
%\includegraphics[width=6cm]{figures_new/regular_blocking/unresolved/fig_1}
%\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases. (Blocking)}
%\label{fig:regular_res_unres_p_blocking}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=7cm]{figures_new/regular_blocking/fig_1}
%\caption{Comparison among the pressure profiles along the line $\rm{A-A^{\prime}}$ for test cases $res_3$, $unres_3$, and the reference solution (Blocking).}
%\label{fig:comparison_res_unres_p_blocking}
%\end{figure}



\begin{table}[ht!]
\caption{Parameters Setting for conductivity and porosity}
\centering
\begin{tabular}{ |p{4cm}||p{1cm}|}
 \hline
 \multicolumn{2}{|c|}{Parameters Values} \\
 \hline
matrix conductivity $K_{M1}$    &  $1$ \\
fracture conductivity $K_{F}$     &   $10^{4}$ \\
matrix porosity$\phi_{M1}$    & $0.2 $ \\
fracture porosity$\phi_{F}$      & $0.2$\\
 \hline
\end{tabular}
\label{tab:param_3}
\end{table}



\begin{figure}[hbt!]
\centering
\includegraphics[width=10cm]{figures_new/small_features/small_feat_geo}
\caption{Geometry Setup and Boundary Conditions (top). Fracture Network (Bottom).}
\label{fig:small_feat_p_1_2_res}
\end{figure}



\begin{figure}
\centering
\subfloat[Unresolved case 1]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea1grid.png}}
\subfloat[Unresolved case 2]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea2grid.png}}\\
\subfloat[Unresolved case 3]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea4grid.png}}
\subfloat[Unresolved case 4]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea6grid.png}}
\label{mesh_unreolved}
\end{figure}

\begin{table}[ht]
\caption{Mesh Setting}
\centering
\begin{tabular}{ |p{2cm}||p{2cm}|p{2cm}|p{2cm}|  }
 \hline
 \multicolumn{4}{|c|}{Resolved Mesh} \\
 \hline
          &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# layers\\
 \hline
$\mathrm{res_1}$    &     3823   &     19964 & 1\\ 
$\mathrm{res_2}$    &      28519   &     159712  & 2\\
$\mathrm{res_3}$    &      220325   &    1277696  &  3\\
$\mathrm{res_4}$    &   1732172   &    10221568 &  4\\
 \hline
 \multicolumn{4}{|c|}{Unresolved Mesh} \\
  \hline
          &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# layers\\
 \hline
$\mathrm{unres_1}$    &      667672  &      560290 & ~1\\ 
$\mathrm{unres_2}$    &           964549   &      933120  & ~2\\
$\mathrm{unres_3}$    &     18634058   &    16727570  &  ~3\\
$\mathrm{unres_4}$    &     90026102  &     84703700 &  ~6\\
 \hline
\end{tabular}
\label{tab:mesh_3}
\end{table}

\subsection{Small Features}
%\begin{enumerate}
%\item  we observe a slow convergence for both the resolved and the unresolved case. Jump in the values used for the constitutive parameters and  for the neumann boundary conditions  affect the regularity of the solution and (The regularity of  the solution is less than $H^2$). A priori, both these issues reduce the convergence rate of the FE method, as the sol must be at least $p-1$ in order to converge with order $p$. The reduction of the convergence rate  due to the jump in the parameters can be avoided with a mesh that resolves the boundary of the discontinuity. In this case, we may get the expected order of convergence. Instead, the problem related to the  discontinuities in the values used for the boundary conditions can not be avoided in any way with the standard continuous fe methods. Possible solutions are to use methods GFEM or multiscale that add special functions to the type of discontinuity, or try to make AMR near the region where boundary conditions changes occur. (Maybe we can mention this also for the regular case)
%\item for the plots over region one may notice a good agreement between the resolved and the unresolved case. Can we say the same also for the pressure?
%\end{enumerate}

\begin{figure}
\centering
\subfloat[a)Spatial  distribution of the pressure]{\includegraphics[width=10cm]{figures_new/small_features/p_small_feat_1}}\\
\subfloat[b) Spatial  distribution of the pressure in the planes $x=0.5$ and $z=0.5$ where line $A-A^{\prime}$ and $B-B^{\prime}$ lie]{\includegraphics[width=10cm]{figures_new/small_features/p_small_feat_2}}
\label{fig:small_feat_p_unres}
\end{figure}




\begin{figure}
\centering
\includegraphics[width=6cm]{figures_new/small_features/resolved/fig_1}
\includegraphics[width=6cm]{figures_new/small_features/resolved/fig_2}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_p_1_2_res}
\end{figure}


\begin{figure}[hbt!]
\centering
\includegraphics[width=6cm]{figures_new/small_features/unresolved/fig_1}
\includegraphics[width=6cm]{figures_new/small_features/unresolved/fig_2}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_p_1_2_unres}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=6cm]{figures_new/small_features/fig_1}
\includegraphics[width=6cm]{figures_new/small_features/fig_2}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_comp}
\end{figure}
\begin{figure}[hbt!]
\hspace{-0.8cm}\includegraphics[width=14cm]{figures_new/small_features/fig_3}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_conc}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=8cm]{figures_new/small_features/c_small_feat}
\caption{Concentration at last time step.}
\label{fig:small_feat_c_ures}
\end{figure}




This benchmark allows for testing the accuracy of the proposed method in the presence of small geometric features. The matrix background is a box $M=(0\,;\,1)\times(0\,;\,2.25)\times(0\,;\,1)\, m$, containing eight fractures.
These are defined by their vertexes and described in~\cite{flemisch2018benchmarks}. The inlet and the outlet are defined as follows: $\partial \Omega_{in}=(0\,;\,1)\times(0)\times(1/3\,;\,2/3)\,m$, $\partial \Omega_{out,1}=(0\,;\,1)\times(2.25)\times(0\,;\,1/3)\,m$,
$\partial \Omega_{out,2}=(0\,;\,1)\times(2.25)\times(1/3\,;\,2/3)\,m$. 

For the flow problem, a uniform inflow on the inlet such that $\int_{\partial \Omega_{in}}\mathbf{u}\cdot \mathbf{n}\,d\gamma=-1/3$, whereas homogeneous Dirichlet boundary conditions are applied on the outlet $\partial \Omega_{out}=\partial \Omega_{out,1}\cup\partial \Omega_{out,2}$. No flow (Neumann) boundary conditions are set on the other boundaries. 

For the transport problem, a Dirichlet boundary condition is imposed on the inlet: $c_{in}=1.0\,m$.
The overall simulation time is set equal to $t_f=10^{2}\,s$ while the time step is set equal to$dt=0.01$.  All the material parameters are summarized in table~\ref{tab:param_3}:


Table ~\ref{tab:mesh_1} lists the number nodes and elements for all performed test cases. As an example, in Figures \ref{mesh_unreolved} and ~\ref{p_small_feat_2} we show the meshes obtained by adopting the adaptive refinement to model the fracture network geometry for all the unresolved test cases reported in Table ~\ref{tab:mesh_1}, and the spatial distribution obtained for test case $\rm{unres}_3$ . In particular ~\ref{p_small_feat_2} b) depicts the spatial distribution of the pressure at planes $x=0.5$ and $z=0.5$ and the extreme points $A=(0.5,\,1.1,\,0)-A^{\prime}=(0.5,\,1.1,\,1)$, and $B=(0,\,2.15,\,0.5)-B^{\prime}=(1,\,2.15,\,0.5)$ of the lines along which the pressure profiles are analized.

Figures~\ref{fig:small_feat_p_1_2_res} and ~\ref{fig:small_feat_p_1_2_unres} depict the pressure profile along the line $A-A^{\prime}$ and $B-B^{\prime}$, for the resolved and the unresolved test cases reported in Table~\ref{tab:mesh_3}. 
We observe that the accuracy of the solution strongly depends on the mesh size for all the performed numerical simulations. 
Figure~\ref{fig:small_feat_comp} shows a comparison between the test cases $\rm{res_4}$ and $\rm{ures_4}$. Small discrepancies can be appreciated since mesh converge was observed neither for the unresolved nor for the resolved test case.

In this regard, it is worth mentioning that the jumps in the values used for the constitutive parameters and the Neumann boundary conditions affect the regularity of the solution. A priori, both these issues reduce the convergence rate of the FE method, as the sol must be at least $p-1$ to converge with order $p$. The reduction of the convergence rate due to the jump in the parameters can be avoided with a mesh that resolves the boundary of the discontinuity. In this case, we may get the expected order of convergence. Instead, the problem related to the discontinuities in the values used for the boundary conditions can not be avoided in any way with the standard continuous Finite Element  Methods. Possible solutions are to use methods GFEM or multiscale that add special functions to the type of discontinuity or try to make AMR near the region where boundary conditions changes occur.
Finally, we analyze the average concentration in each fracture and plot the results in Figure~\ref{fig:small_feat_conc} which reveals a good agreement between the test cases $\rm{res_4}$ and $\rm{ures_4}$. Indeed, as one may observe
figures~\ref{fig:small_feat_p_1_2_res} and ~\ref{fig:small_feat_p_1_2_unres}, the progressive refinement performed to solve for the flow problem, produces as the main effect the sum of a constant to the coarsest solution. Hence, even though the values of the pressure field increase,  the computation of the corresponding gradient, and consequently of the velocity field, will produce similar results.







\subsection{Hydrocoin}
%\begin{enumerate}
%\item good agreement between unresolved and the reference solution
%\end{enumerate}
This flow problem was presented within the international Hydrocoin project, (Swedish Nuclear Power Inspectorate (SKI) and proposed as benchmark for both hybrid and equi-dimensional models in~\cite{flemisch2018benchmarks}. Concerning the boundary conditions,  a piezometric head is imposed on the top boundary of the domain, whereas  no  flow (Neumann) boundary conditions are set on the other boundaries. We only consider the unresolved test case consisting of $12683$ elements and $10938$ nodes and compare the corresponding solution for the pressure with the reference  solution obtained by a standard FV method on a continuous fracture model and computed on a grid with $3 527 296$
elements and $3 813 249$ nodes ~\cite{flemisch2018benchmarks}. 
\begin{table}[htb!]
\caption{Parameters Setting for conductivity and porosity}
\centering
\begin{tabular}{ |p{4cm}||p{1cm}|}
 \hline
 \multicolumn{2}{|c|}{Parameters Values} \\
 \hline
matrix conductivity $K_{M}$    &  $10^{-8}$ \\
fracture conductivity $K_{F}$    &  $10^{-6}$ \\
 \hline
\end{tabular}
\label{tab:param_1}
\end{table}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm ]{figures_new/hydro}
\caption{Benchmark 1. Locally refined mesh with Ndof equato to 259600 (AMR$_5$). Fractures are represent by means an AME techniques,}
\label{fig:setup_hydro}
\end{figure}
\begin{figure}[ht]
\centering
\includegraphics[width=7cm]{figures_new/hydrocoin/fig}
\caption{Pressure profiles for  the benchmark \textit{hydrocoin} along the line $A-A^{\prime}$ }
\label{fig:hydro_p}
\end{figure}


Figure~\ref{fig:setup_hydro} shows the pressure distribution and the extreme points of  $A=(0\,;\,-200\,;\,0)$ and $A^{\prime}=(1600\,;\,-200\,;\,0)$ of the line along which the pressure is analyzed.  In Figure~\ref{fig:hydro_p}, we observe a good agreement between the numerical results obtained for the unresolved test case and the reference solution.


\subsection{Realistic}

In this last test case, we consider a real set of fractures from an interpreted outcrop in the Sotra island, near Bergen in Norway. The set comprises
64 fractures grouped in 13 different connected networks, ranging from isolated fractures up to tens of fractures each. In the interpretation process, two fractures are composed of more than one segment. The size of the domain is $700\,m \times 600 \,m$ with uniform matrix permeability $K_m = 10$. For simplicity, all the fractures have the same scalar permeability $K_f=10^{-6}$. Concerning the boundary conditions, we consider homogeneous Neumann boundary conditions (no flow) on the top and bottom side, a pressure $P= 1013250\,[Pa]$ is applied on the left side, and pressure $P=0\,[Pa]$ on the right side of the domain.
In Figure~\ref{fig:realistic_line_1} we analize the mesh converge by analyze the pressure along the lines $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for all the unresolved test cases reported in Table~\textbf{add table}.
While we observe that all the pressure profiles show similar behavior, relevant differences are found in the pressure distribution reported in Figure~\ref{fig:realistic_pressure} where a similar pattern is only observed for the test cases $\rm{unres_3}$ and $\rm{unres_4}$.
Figure~\ref{fig:realistic_line_1} shows a comparison between our numerical results and those obtained with the numerical methods presented in ~\cite{flemisch2018benchmarks}. Again a good agreement is found among all the profiles. 

\begin{figure}
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh0.pdf}}
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh3.pdf}}\\
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh4.pdf}}
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh6.pdf}}
\end{figure}



\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm]{figures_new/realistic/convergence}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:realistic_line_1}
\end{figure}



\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{figures_new/realistic/fig_realistic_p_tot}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:realistic_pressure}
\end{figure}


\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm]{figures_new/realistic/comparison}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:realistic_line_1}

\end{figure}



\newpage

%\printbibliography





==> sections/05ResultsDMP.tex. <==
\section{Numerical examples}

In this section, we validate the proposed approach using five benchmark cases. The first benchmark is s a two-dimensional version of the test case proposed in~\cite{BenchPaper}
The second benchmark case is based on Geiger et al. (2013) ~\cite{flemisch2018benchmarks} and shows a regular fracture network. The third test case is based on a well-established benchmark for groundwater flow from Swedish Nuclear Power Inspectorate (SKI) (1987). The fourth taste case is a three-dimensional test case containing small geometric features~\cite{BenchPaper}, whereas the last benchmark considers a realistic scenario where several fractures randomly oriented are embedded in a rock matrix.

For each benchmark,  we consider both the resolved and the unresolved test cases and compare the numerical results in terms of pressure and concentration profiles along the prescribed lines.


\subsection{Adaptive mesh refinement\\ for heterogenous media}

In this section, we briefly summarize the AMR method, whose details are presented in \cite{Holliger2000}.
The idea at the base is to start with a coarse uniform mesh.
In particular, for cuboid domains of tipe $\Omega^c$,
the initial mesh can also be thought as structured.
The initial mesh is not supposed to explicitly resolved the interfaces between the background and the fractures.

Then, given a distribution of embedded fractures,
we iterate over all elements and mark for refinement the ones that have non-empty intersections with the boundary of at least one fracture.

In some cases, it can be useful to change the target according to which we decide to mark for refinement.
For example, when conductive fractures are considered, i.e., fractures which have a permeability much larger compared to the one of the matrix,
it is convenient to mark for refinement all the elements that have a non-empty overlap with at least one fracture.
This means that elements insides a fracture are refined as well.
Moreover, the refinement region can be a region around the fracture but not necessarily coinciding with the fracture.


This procedure allows to create a sequence of meshes, which become progressively finer towards the interfaces.
This AMR method allows to automatically create meshes for any heterogeneity distribution without any human interaction.
In order to keep the meshes $1$-irregular, at each step the refinement region may be enlarged in order to satisfy such a constraint.


%In order to evaluate the accuracy of the method, solutions or output variables, such as seismic attenuation and velocity dispersion,
%from two consecutive hierarchical levels can be compared.

%Another possibility for evaluating the quality of the solution would be to employ error estimators,
%which are not readily available for the proposed method.
%In this regard, there are basically two options.
%One would be to adapt error estimators based on flux reconstruction that have already been developed for Biot's equations in the time domain \cite{RIEDLBECK20171593}.
%Here, the main difficulty would be to extend this methodology to complex vector spaces and non-symmetric problems.
%Another would be to use more generic residual-based error estimators for coupled problems, e.g. \cite{ern2009posteriori}.


\subsection*{Resolved and unresolved discretizations}
We finally introduce two different methods to simulate flow and transport in fractured media.

\textit{Resolved discretization} The first discretization will be referred to as \emph{resolved} and its meshes resolve the interfaces between the matrix and the fractures. It makes use of conforming meshes which are, in general, complicated to generate,
since they require a lot of human-computer interaction to achieve the desired mesh quality. The mesh generation of a fractured network system is usually tedious and difficult  to make automatic due to the geometric complexity of the computational domain induced by existence and extension of fractures.

\textit{Unresolved discretization} The second discretization will be referred to as \emph{unresolved} and its meshes do not explicitly resolve the interfaces between the matrix and the fractures,
but are actually refined close to such interfaces. More specifically an adaptive refinement procedure is adopted to ensure the desired leyer of elements inside  each fracture network. Given a mesh $\mathcal{T}$, each element is initially marked as belonging to either the background matrix or to the fracture network. Then all the elements marked as \textit{fractured} are progressively refined until the desired mesh-accuracy is achieved.

\textbf{Remark} For the unresolved discretization, all the bilinear and linear operators, i.e matrices and vectors, are computed element-wise on the non-conforming space $W^H$ and them projected onto the regular space $V^r$ by means of the interpolation operator~\eqref{eq:interp}.

It is worth to pointing out that, the stabilization of the transport problem can be also either performed on the  transport operator $\mathbf{A}$ or on its element-wise contribution $[\mathbf{A}]_{ij}$ . While there is no difference between the two approaches when conforming meshes are adopted, the use of non-conforming meshes makes mandatory the first approach. Indeed, if one stabilize the local contribution $[\mathbf{A}]_{ij}$, the subsequent use of the relation $\eqref{eq:intA}$ introduces off diagonal entries which violate the assumptions 1a and 1b of theorem~\ref{th:DM} needed to ensure the DMP.

According to the definitions above, a triangulation can be non-conforming and non-uniform but all elements are shape-regular, being squares or cubes.



%\textbf{It is also a very tedious task to create a full-dimensional description of the fracture network and a corresponding equi-dimensional grid of the whole computational domain. Therefore, we refrain from calculating a reference solution with the MFD method and per- form a direct comparison of the hybrid-dimensional methods.
%It is also a very tedious task to create a full-dimensional description of the fracture network and a corresponding equi-dimen- sional grid of the whole computational domain. Therefore, we refrain from calculating a reference solution with the MFD method and per- form a direct comparison of the hybrid-dimensional methods..}

%Ciò che inficia la regolarità sono i jump nei parametri (mi sembra che la sol appartenga a H^5/4) e particolari cambi di boundary conditions (La sol è meno di H^2). A priori entrambi questi problemi riducono la convergenza dei metodi fe, in quanto la sol deve essere almeno in p+1 al fine di avere convergenza con ordine p. Il converence rate ridotto dovuto ai jump nei parametri può essere evitato con mesh che risolvono i boundary delle discontinuità. In questo caso si ottengono ordini di convergenza simili al problema senza discontinuità, con il fatto che se ci sono molte discontinuità sono difficili da meshare. Invece il problema legato alla discontinuità del tipo di boundary conditions non può essere evitato in alcun modo con i fe standard. Possibili soluzioni sono usare metodi GFEM o multiscala che aggiungono particolari funzioni legate al tipo di discontinuità oppure provare a fare AMR vicino al cambio del tipo di boundary conditions.}


\subsection{Single 2D}
%\begin{enumerate}
%\item good agreement between unresolved and resolved
%\item for the resolved case meshes comprising poor-quality elements may affect the accuracy of the method as shown in Figure~2
%\end{enumerate}
The first benchmark example consists of a square-shaped domain $\Omega_{M}$ crossed by a an oblique fracture $\Omega_{F}$ with a thickness $\delta=0.01$. To represent an heterogeneous rock matrix, different material properties are assigned to a sub-domain $\Omega_{het}$ defined in lower part of the domain $M$.  A geometrical description of the rock matrix and the fracture are depicted in Figure, whereas more details on the geometrical sizes can be found in Table~\ref{tab:geo_1}.
\begin{table}[ht]
\caption{Geometrical sizes}
\centering
\begin{tabular}{ |p{1cm}||p{1cm}|p{1cm}|p{1cm}| |p{1cm}|  }
 \hline
 \multicolumn{5}{|c|}{Rock Matrix} \\
 \hline
      & {$\bf{x_{s}}$} [m]& $\bf{x_{e}}$ [m]& $\bf y_{s}$ [m]& $\bf y_{e}$ [m] \\
 \hline
$\mathrm\Omega_{M}$ &-50 & 50 & -50 & 50    \\
$\mathrm\Omega_{het}$  &-50 & 50 & -50 & -40  \\
$\mathrm{\Gamma_{in}}$  &0 & 0 & 40 & 50  \\
$\mathrm{\Gamma_{out}}$  &50 & 50 & 0 & 10  \\
 \hline
 \multicolumn{5}{|c|}{Fracture} \\
  \hline
      & $ \bf x_{s}$ [m]& $\bf x_{e}$ [m]& $\bf y_{s}$ [m]& $\bf y_{e}$ [m]  \\
 \hline
 $\mathrm\Omega_{F}$& -50   & 50 & -30 & 30\\
 \hline
\end{tabular}
\label{tab:geo_1}
\end{table}

Concerning the boundary conditions, for the flow problem, we impose a Dirichlet condition at the inlet $\Gamma_in$ with $p_{in}^{D}= 4m$ and at the outlet $\Gamma_{out}$ with $p_{out}^{D} = 1m$,  whereas for the transport problem, we impose a Dirichlet condition $c_{in}^{D} = 0.01m^{2}$ at the inlet $\Gamma_{in}$.  For the transport problem, the overall simulation time is $t_f=10^{9}\,\rm{[s]}$ and the time step is $dt=10^2~\rm{[s]}$. The parameters adopted for the material properties are summarized in Table~\ref{tab:geo_1}. 


\begin{table}[ht]
\caption{Parameters Setting for conductivity and porosity}
\centering
\begin{tabular}{ |p{4cm}||p{1cm}|}
 \hline
 \multicolumn{2}{|c|}{Parameters Values} \\
 \hline
matrix conductivity $\bf K_{M1}$    &  $10^{-6}$ \\
matrix conductivity $\bf K_{M2}$    &  $10^{-5}$ \\
fracture conductivity $\bf K_{F}$     &   $10^{-1}$ \\
matrix porosity$\boldsymbol{\phi_{M1}}$    & $0.2 $ \\
matrix porosity $\boldsymbol{\phi_{M2}}$   & $0.2$  \\
matrix porosity $\boldsymbol{\phi_{M3}}$   &  $0.25$ \\
fracture porosity$\boldsymbol{\phi_{F}}$      & $0.4$\\
 \hline
\end{tabular}
\label{tab:param_1}
\end{table}

Four different meshes are considered for the resolved and the unresolved configurations. In Table~\ref{tab:mesh_1} we report the number of nodes, elements and layer of elements inside the fracture for each test case. 
\begin{figure}[hbt!]
\centering
\includegraphics[width=9cm]{figures_new/single/fig_mesh_unres}
\caption{Locally refined mesh for the test case $\rm{unres_3}$. }
\label{fig:single_unresolved_mesh}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm ]{figures_new/single_p}
\caption{Pressure distribution for the test case $\rm{unres_3}$ (Units [Pa]).}
\label{fig:single_p_unresolved_setup}
\end{figure}

%\begin{figure}[hbt!]
%\centering
%\hspace{0.1cm}
%\includegraphics[width=11cm ]{figures_new/single/single_c_tot}
%\caption{Concentration distribution at time $t=2\,10^{8}[s]$ and $t=\,10^{9}[s]$ for the test case $\rm{unres_3}$ (Units [m]).}
%\label{fig:unresolved_single_c}
%\end{figure}

As an example, in Figures~\ref{fig:single_unresolved_mesh}, \ref{fig:single_p_unresolved_setup} and~\ref{fig:unresolved_single_c} we show  the mesh used for the test case $\mathrm{unres_3}$,   the corresponding solution obtained by solving the flow problem, and  the one resulting from the transport problem, respectively. In particular, we in Figure~\ref{fig:unresolved_single_c} we show the concentration distribution at the time instants $t=2\,10^{8}[s]$ and $t=\,10^{9}[s]$.  The obtained results confirm the ability of  stabilization technique to preserve the positivity of the solution and ensure the local maximum principle.


\begin{table}[ht]
\caption{Mesh Setting for Benchmark Single 2D}
\centering
\begin{tabular}{ |p{2cm}|p{2cm}|p{2cm}|p{1cm}|p{2cm}|p{2cm}|  }
 \hline
 \multicolumn{6}{|c|}{Resolved Mesh} \\
 \hline
      &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
$\mathrm{res_1}$&\,\,\,\,\,\,\,6\,785  &\,\,\,\,\,\,\,6\,612 &  1& $1.86675\,e^{-6}$  & $-1.86675\,e^{-6}$\\
$\mathrm{res_2}$&\,\,\,26\,793  &\,\,\,\,26\,448 &  2& $1.85977\,e^{-6}$  & $-1.85977\,e^{-6}$\\
$\mathrm{res_3}$& 106\,481  & 105\,792 &  3& $1.85632\,e^{-6}$  & $-1.85632\,e^{-6}$\\
$\mathrm{res_4}$& 424\,545  & 423\,168 &  4& $1.85457\,e^{-6}$  & $-1.85457\,e^{-6}$\\
 \hline
 \multicolumn{6}{|c|}{Unresolved Mesh} \\
  \hline
        &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
 $\mathrm{unres_1}$&\,\,\,\,162\,628   &\,\,\,\,141\,640  & 1.28  & $1.86277\,e^{-6}$ & $-1.86277\,e^{-6}$\\
  $\mathrm{unres_2}$&\,\,\,\,401\,680   &\,\,\,\,442\,813  & 2.56  & $1.85779\,e^{-6}$ & $-1.85779\,e^{-6}$\\
 $\mathrm{unres _3}$&1\,291\,360      &1\,375\,252 & 5.12       &$1.85534\,e^{-6}$ & $-1.85534\,e^{-6}$ \\
 $\mathrm{unres _4}$&2\,678\,304      &2\,512\,480 &10.24      & $1.85517\,e^{-6}$ & $-1.85517\,e^{-6}$ \\
 \hline
\end{tabular}
\label{tab:mesh_1}
\end{table}




\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/single/conservation}
\caption{Flux conservation}
\label{fig:single_flux}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/single/pressure}
\caption{Pressure Profile}
\label{fig:single_P}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/single/concentration}
\caption{Concentration}
\label{fig:single_CM}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=8cm]{figures_new/single/fig_mesh_res}
\caption{Left: mesh of the test case $\rm{res_{1,\rm{uni}}}$ together with a zoom-in of the region close to end point $\rm B^{\prime}$. Right: comparison between  the concentration profiled obtained for the test cases $\rm{res_{1,\rm{uni}}}$  and  $\rm{res_1}$ along the line $\rm{B-B^{\prime}}$.}
\label{fig:mesh_c_recolved_bench_1}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/single/concentration_correction_2}
\caption{Concentration distribution at time $t=2\,10^{8}[s]$ and $t=\,10^{9}[s]$ for the test case $\rm{unres_3}$ (Units [m]).}
\label{fig:unresolved_single_c}
\end{figure}

%\begin{figure}[hbt!]
%\includegraphics[width=6cm]{figures_new/single/resolved/fig_1}
%\includegraphics[width=6cm]{figures_new/single/unresolved/fig_1}
%\caption{Pressure profiles along the line $\rm{A-A^{\prime}}$ for all the resolved (left) and unresolved (right) cases presented in Table~\ref{tab:mesh_1}. }
%\label{fig:figure_p_res_unres_bench1}
%\end{figure}
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=7cm]{figures_new/single/fig_1}
%\caption{Pressure profiles along the line $\rm{A-A^{\prime}}$ for the finest resolved and unresolved test cases, respectively.}
%\label{fig:figure_p_comp_bench1}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/single/resolved/fig_2}
%\includegraphics[width=6cm]{figures_new/single/unresolved/fig_2}
%\caption{Concentration profiles  at final time along the line $\rm{A-A^{\prime}}$ for all the resolved (left) and unresolved (right) cases presented in Table~\ref{tab:mesh_1}. }
%\label{fig:figure_c1_bench1}
%\end{figure}


%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/single/resolved/fig_3}
%\includegraphics[width=6cm]{figures_new/single/unresolved/fig_3}
%\caption{Concentration profiles  at final time along the line $\rm{B-B^{\prime}}$ for all the resolved (left) and unresolved (right) cases presented in Table~\ref{tab:mesh_1}.}
%\label{fig:figure_c2_bench1}
%\end{figure}
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/single/fig_3}
%\includegraphics[width=6cm]{figures_new/single/fig_2}
%\caption{Concentration profiles  at time $t=t_f$ along the line $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for the finest resolved and the unresolved test case, respectively.}
%\label{fig:figure_c_comp_bench1}
%\end{figure}







We validate our approach by analyzing the pressure and the concentration profiles along the lines connecting the points $\rm{A-A^{\prime}}$, with coordinates $\rm{A}=(50;-50;0)$, and $\rm{A^{\prime}}=(-50;50;0))$, and $\rm{B-B^{\prime}}$, with coordinates $\rm{B}=(30;-30;0)$, and $\rm{B^{\prime}}=(-30;30;0))$, as depicted in Figure~\ref{fig:single_p_unresolved_setup}.

In Figures~\ref{fig:figure_p_res_unres_bench1} and~\ref{fig:figure_p_comp_bench1} we compare the pressure computed along the line $\rm{A-A^{\prime}}$ for all the test cases presented in Table~\ref{tab:mesh_1}. No relevant differences are found among all the numerical results (Figure~\ref{fig:figure_p_res_unres_bench1}) and a good agreement is observed between the resolved and the unresolved solution (Figure~\ref{fig:figure_p_comp_bench1}).


In Figures~\ref{fig:figure_c1_bench1} and ~\ref{fig:figure_c2_bench1} the concentration obtained at time $t=t_f$ along the lines $\rm{A-A^{\prime}}$ and  $\rm{B-B^{\prime}}$ is plotted. Again, all the analyzed profiles reveal a similar behaviour and a good match is found between the resolved and the unresolved results, as shown in Figure~\ref{fig:figure_c_comp_bench1}.

It is worth pointing out that the use of adaptive refinement allows controlling the quality of the mesh which represents an important requirement to ensure the stability of the method and accuracy of the solution. In this regard, in Figure~\ref{fig:mesh_c_recolved_bench_1} we show a comparison between the concentration obtained for the test cases $\rm{res_{1,\rm{uni}}}$ and $\rm{res_1}$ along the line $\rm{B-B^{\prime}}$. Differences can be clearly observed close to the endpoint $\rm{B^{\prime}}$ and are mainly related to the poor-quality of the mesh $\rm{res_{1,\rm{uni}}}$ obtained by performing one uniform refinement step on the mesh used for the test case $\rm{res_{1}}$.




\subsection{Regular}
%\begin{enumerate}
%\item good agreement between unresolved and resolved
%\item for the unresolved we observe a deviation the solution along line 2 whereas along line 1 (fracture in the middle) we get good match for both the resolved the unresolved meshes.
%Can we justify the deviation with the low order of convergence due to the discontinuity in both parameters and boundary conditions? this hypothesis seems to be supported from the fact that in the blocking case we get good agreement with respect to the reference solution for both resolved and the unresolved mesh. 
%\item for the concentration can we justify the differences between the resolved and the unresolved case in the same way as done for the pressure?
%\item for the plots over region the concentration seems to tend to zero in regions 2 4 and 6 (figure 18). The diffusion added by the stabilization term seems to prevent the solution to go to zero (shell we mention this?). Can  we refer to the  differences between the solutions in these regions to justify also the differences obtained in the plots over line (see figures~15 and 17)?
%\end{enumerate}

The second benchmark consists of a regular fracture network embedded in square with size $x_s=0\,m\,x_e=1\,m$ and $y_s=0\,m\,y_e=1\,m$. The rock has a unitary conductivity $K_M = I$, whereas for the fractures we consider two cases: a highly conductive fracture network with $K_F = 10^4$ and a blocking fracture network with $K_F=10^{-4}$. For the transport problem, the matrix and the fracture network have the same porosity,~i.e. $\phi_m=\phi_f=1.0$.

For the flow problem, we apply homogeneous Neumann conditions (no flow) on top and bottom sides, a unitary inflow flux $u_N=-1$ on the left boundary, and a Dirichlet condition $p_D = 1$ on the right boundary. Our numerical results are compared with the numerical approaches and the reference solution presented in~\cite{flemisch2018benchmarks}. 

For the transport problem, a unitary concentration $c_d=1.0$ is imposed on the left boundary, whereas homogeneous Neumann conditions (no flow) are applied on the remaining sides.  The time step $dt=0.025~\rm{[s]}$ and the overall simulation time is set equal to$t_f=0.5,~\rm{[s]}$. 





%    \begin{figure}[hbt!]
%    \centering
%    \includegraphics[width=3.8cm]{figures/regular/RegularConfC1.eps}
%    \includegraphics[width=3.8cm]{figures/regular/RegularAMRC1.eps}
%    \includegraphics[width=3.8cm]{figures/regular/RegularConfAMRC1.eps}
%    \caption{Benchmark 2 with conductive fractures: comparison of concentration values along the line $y=0.5$}
%    \label{fig:figure_p1_bench2}
%    \end{figure}

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=3.8cm]{figures/regular/REgularConfC2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularAMRC2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularConfAMRC2.eps}
%\caption{Benchmark 2 with conductive fractures: comparison of concentration values along the line $y=0.5$}
%\label{fig:figure_p1_bench2}
%\end{figure}

% \begin{figure}[hbt!]
% \centering
% \includegraphics[width=8cm]{figures/RegularVerticalLine}
% \caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $x=0.5$.}
% \label{fig:figure_p2_bench2}
% \end{figure}




\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm]{figures_new/regular_p}
\caption{Pressure distribution for the test case $\rm{unres_3}$ (Units [Pa])}
\label{fig:unresolved_regular_p}
\end{figure}


%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=10cm]{figures_new/regular_c_tot}
%\caption{Concentration distribution at time $t=\,0.20[s]$ and $t=\,0.5[s]$ for the test case $\rm{unres_3}$ (Units [m]).}
%\label{fig:unresolved_regular_c}
%\end{figure}

\subsubsection{Conductive fracture network}
First, we consider a highly conductivity network. Three different meshes are considered for the resolved and the unresolved configurations. In Table ~\ref{tab:mesh_2} we report the number of nodes, elements and layer of elements inside the fracture for each test case.

\begin{table}[ht]
\caption{Mesh Setting for Benchmark Regular 2D}
\centering
\begin{tabular}{ |p{2cm}|p{2cm}|p{2cm}|p{1cm}|p{2cm}|p{2cm}|  }
 \hline
 \multicolumn{6}{|c|}{Resolved Mesh} \\
 \hline
      &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
%$\mathrm{unres_0}$&     29929 &   29584    &  4\\
$\mathrm{unres_1}$&   110889 &  110224    &  4&  0.662191 & -0.662191\\
$\mathrm{unres_2}$&   426409 &  425104   &  4 & 0.662189 & -0.662189\\
$\mathrm{unres_3}$&   1671849    & 1669264   &  4 & 0.662185&-0.662185\\
$\mathrm{unres_4}$&    16056049   &   16048036  &  2&  0.662177 & -0.662177\\
 \hline
 \multicolumn{6}{|c|}{Unresolved Mesh} \\
  \hline
      &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
$\mathrm{unres_1}$&  1\,863\,685 &    1\,720\,768    &  4& 0.65692& -0.65692\\
$\mathrm{unres_2}$&     1\,879\,729 &   1\,736\,896  &  4 &0.656915 &-0.656915 \\
$\mathrm{unres_3}$&    4\,673\,031     &  4\,387\,096   &  8 &0.662382 &-0.662382\\
$\mathrm{unres_4}$&      4\,966\,635   &  4\,681\,144   &  8& 0.662381& -0.662381\\
$\mathrm{unres_5}$&        15\,054\,349   &    14\,483\,152   &  16&0.662415&-0.662415\\
 \hline
\end{tabular}
\label{tab:mesh_2}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c| c |}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11\\
80 &  &  &  &  &  &  0.12045&  0.11707&  0.11704&  0.11823&  0.1182 \\
160 &  &  &  &  &  0.12031&  0.11692&  0.11691&  0.11811&  0.11808&   \\
320 &  &  &  &  0.12023&  0.11684&  0.11683&  0.11803&  0.11801&  &   \\
640 &  &  &  0.1202&  0.11679&  0.11679&  0.11799&  0.11797&  &  &   \\
1280 &  &  0.12018&  0.11677&  0.11677&  0.11797&  0.11794&  &  &  &   \\
2560 &  0.12017&  0.11676&  0.11676&  0.11796&  0.11793&  &  &  &  &   \\
\end{tabular}
\caption{flussi unresolved stab}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c| c |}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 \\
80 &  &  &  &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11776 \\
160 &  &  &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&   \\
320 &  &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &   \\
640 &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &  &   \\
1280 &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &  &  &   \\
2560 &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &  &  &  &   \\
\end{tabular}
\caption{flussi unresolved non-stab}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c| c |}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 \\
80 &  &  &  &  &  &  474.29&  951.49&  3537.8&  9321.43&  30687.04 \\
160 &  &  &  &  &  533.79&  997.24&  3541.53&  9293.61&  29055.21&   \\
320 &  &  &  &  825.26&  1305.83&  3817.38&  9345.93&  28419.23&  &   \\
640 &  &  &  1573.17&  2161.3&  4909.56&  10994.99&  29168.34&  &  &   \\
1280 &  &  5397.39&  6343.81&  9328.68&  15453.4&  37212.82&  &  &  &   \\
2560 &  10726.8&  11474.12&  13512.52&  17933.18&  31340.79&  &  &  &  &   \\
\end{tabular}
\caption{solution time non stab, decidi se torna utile}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | }
 & 1 & 2 & 4 & 8 & 16 \\
80 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11775 \\
160 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11775 \\
320 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11775 \\
640 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11776 \\
1280 &  0.11775&  0.11775&  0.11776&  0.11776&  0.11776 \\
\end{tabular}
\caption{flussi resolved}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | }
 & 1 & 2 & 4 & 8 & 16 \\
80 &  44.03&  43.74&  44.56&  33.11&  42.12 \\
160 &  59.9&  67.31&  70.1&  76.72&  96.27 \\
320 &  216.14&  212.6&  220.18&  220.88&  259.91 \\
640 &  844.39&  816.7&  918.61&  888.23&  1007.48 \\
1280 &  3678.56&  3725.55&  3476.15&  3829.14&  3680.57 \\
\end{tabular}
\caption{solution time resolved, direi che non \'e utile}
\end{table}

In Figure~\ref{fig:unresolved_regular_p} we show the spatial distribution of the pressure, and  the extreme points of the lines $A-A^{\prime}$, $(x=0.5)$, and $B-B^{\prime}$, $(y=0.75)$ along which we perform our analysis.
Figures~\ref{fig:regular_p1_res_unres} and ~\ref{fig:regular_p1_res_unres} depict the pressure profile along the line $A-A^{\prime}$ and  $B-B^{\prime}$,  for the resolved and the unresolved test cases reported in Table~\ref{tab:mesh_2}. Here, one may observe that all the solutions exhibit a similar behaviour. Figure~\ref{fig:regular_p1_p2_comp} shows a comparison with the numerical methods and the reference solution presented in ~\cite{flemisch2018benchmarks}. It refers to a very fine reference mesh, with a total of $1\,175\,056$ element, where the fractures are resolved by ten elements in their normal direction.

While all the results reveal a good match for line $A-A^{\prime}$, a small deviation is found for the test case $\rm{unres_3}$ along the line $B-B^{\prime}$, where our method shows a good agreement with the Embedded Discrete Fracture Method (EDFM).
\begin{table}[ht]
\caption{List of Regions}
\centering
\begin{tabular}{ |p{2cm}||p{2cm}|p{2cm}|  }
 \hline
      & $\mathbf{x}_{range}$    & $\mathbf{y}_{range}$ \\
       \hline
$\mathrm{1}$&  [0\,\,0.5] &   [0\,\,0.5]   \\
$\mathrm{2}$&   [0.5\,\,1.0] &   [0\,\,0.5]   \\
$\mathrm{3}$&  [0\,\,0.5]     &  [0.5\,\,1.0]    \\
$\mathrm{4}$&  [0.75\,\,1.0]     &  [0.75\,\,1.0]    \\
$\mathrm{5}$&  [0.75\,\,1.0]     &  [0.5\,\,0.75]    \\
$\mathrm{6}$&  [0.5\,\,0.75]     &  [0.75\,\,1.0]    \\
$\mathrm{7}$&  [0.5\,\,0.625]     &  [0.5\,\,0.6250]    \\
$\mathrm{8}$&  [0.625\,\,0.75]     &  [0.5\,\,0.6250]    \\
$\mathrm{9}$&  [0.5\,\,0.6255]     &  [0.625\,\,0.6250]    \\
$\mathrm{10}$&  [0.625\,\,0.75]     &  [0.625\,\,0.750]    \\
 \hline
\end{tabular}
\label{tab:regions}
\end{table}
In Figures~\ref{fig:c1_regular_res_unres} and~\ref{fig:c2_regular_res_unres}, we compare the concentration at the final time $t=t_f$ along the lines $\rm{B-B^{\prime}}$ and $\rm{C-C^{\prime}}$($y=0.5$ in Figure~\ref{fig:unresolved_regular_p}),respectively. We can observe mesh convergence for both the resolved and the unresolved test cases. In particular, while a good agreement is found among all the results related to the unresolved configuration, we observe that the difference among the solutions computed for the resolved test cases progressively reduces with mesh refinement. 
A comparison between the resolved and the unresolved test cases is performed by analyzing both the concentration along lines $B-B^{\prime}$ and $C-C^{\prime}$ and the average concentration in the regions listed in Table~\ref{tab:regions}. The two configurations reveal a good agreement for all the regions except for region $2$ where the solution obtained for the unresolved case $\rm{unres_3}$ is almost half the one computed for the resolved one $\rm{res_3}$. However, we have observed that the concentration in this region progressively decreases by uniformly refining the grid (not shown). Thus, we believe that the differences between the numerical solutions are mainly related to the artificial diffusion introduced by the stabilization which prevents the concentration to become zero.

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_res_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_unres_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_tot}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}


\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_u_r}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/cm_res_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/cm_ures_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/regular/cm_res_vs_ures_1}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/regular/cm_res_vs_ures_2}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/regular/cm_res_vs_ures_3}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures/fig_single_4}
%\includegraphics[width=8cm]{figures/fig_mesh_2}
%\caption{Concentration profiles for the benchmark \textit{single2d}  at final time along the fracture $(50\,;\,-30\,;\,0), (-50\,;\,30\,;\,0)\,m$ for the test case 4.}
%\label{fig:figure_c3_bench1}
%\end{figure}

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_3.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_4.eps}
%\caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the lines $x=0.5$ and $y=0.7$ for different conformed-mesh size}
%\label{fig:regular_p1_unres}
%\end{figure}

\clearpage

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_1.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_1.eps}
%\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
%\label{fig:regular_p1_res_unres}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_2.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_2.eps}
%\caption{Pressure along the line $B-B^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases. (Conductive)}
%\label{fig:regular_p1_res_unres}
%\end{figure}
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/fig_1}
%\includegraphics[width=6cm]{figures_new/regular/fig_2}
%\caption{Comparison among the pressure profiles along the lines $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for test cases $res_3$, $unres_3$, and the reference solution (Conductive).}
%\label{fig:regular_p1_p2_comp}
%\end{figure}

\clearpage

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=3.8cm]{figures/regular/RegularConfP1.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularAMRp1.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularVerticalLine}
%\caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $x=0.5$ for different conformed-mesh size}
%\label{fig:figure_conf_bench2}
%\end{figure}

% \begin{figure}[hbt!]
% \centering
% \includegraphics[width=8cm]{figures/RegularAmr}
% \caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $x=0.5$ for different AMR-mesh size}
% \label{fig:figure_amr_bench2}
% \end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=3.8cm]{figures/regular/RegularConfp2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularAMRp2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularHorizontalLine.png}
%\caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $y=0.7$}
%\label{fig:figure_p1_bench2}
%\end{figure}


%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_3.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_5.eps}
%\caption{Concentration at final time $t=0.5~[s]$ along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
%\label{fig:c1_regular_res_unres}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_4.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_6.eps}
%\caption{Comparison among the concentration profiles along the lines $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for test cases $res_3$, $unres_3$ (Conductive).}
%\label{fig:c1_c2_regular_res_unres}
%\end{figure}
%
%
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/fig_3}
%\includegraphics[width=6cm]{figures_new/regular/fig_4}
%\caption{Concentration at final time $t=0.5~[s]$ along the line $B-B^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
%\label{fig:c2_regular_res_unres}
%\end{figure}
%
%
%
%
%\begin{figure}[hbt!]
%\hspace{-0.8cm}\includegraphics[width=12cm]{figures_new/regular/fig_5}
%\caption{Average concentration in the regions defined in~\ref{tab:regions} over time (Conductive).}
%\label{fig:figure_c_bench2}
%\end{figure}
%
%
%\subsubsection{Blocking fracture network}
%We now present the numerical results obtained for the blocking fracture network. In particular, we focus on the comparison between the numerical results obtained by solving the flow problem on the resolved and the unresolved meshed reported in Table~\ref{tab:mesh_2}. As an example, the pressure distribution is shown in Figure~\ref{fig:regular_blocking_p} where 
%one may observe the pressure discontinuities induced by the low fracture permeability.
%Figures~\ref{fig:regular_res_unres_p_blocking} and ~\ref{fig:comparison_res_unres_p_blocking} depict the pressure profile along the line $\rm{A-A^{\prime}}$, with coordinated $A=(0.1,0,0)$ and $A^{\prime}=(1.0,0.9,0)$ . Again a good agreement is found among all the numerical solutions.
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=7cm]{figures_new/regular_p_blocking_2}
%\caption{Pressure distribution for unresolved test case $\rm{unres_3}$ (Blocking).}
%\label{fig:regular_blocking_p}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular_blocking/resolved/fig_1}
%\includegraphics[width=6cm]{figures_new/regular_blocking/unresolved/fig_1}
%\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases. (Blocking)}
%\label{fig:regular_res_unres_p_blocking}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=7cm]{figures_new/regular_blocking/fig_1}
%\caption{Comparison among the pressure profiles along the line $\rm{A-A^{\prime}}$ for test cases $res_3$, $unres_3$, and the reference solution (Blocking).}
%\label{fig:comparison_res_unres_p_blocking}
%\end{figure}



\begin{table}[ht!]
\caption{Parameters Setting for conductivity and porosity}
\centering
\begin{tabular}{ |p{4cm}||p{1cm}|}
 \hline
 \multicolumn{2}{|c|}{Parameters Values} \\
 \hline
matrix conductivity $K_{M1}$    &  $1$ \\
fracture conductivity $K_{F}$     &   $10^{4}$ \\
matrix porosity$\phi_{M1}$    & $0.2 $ \\
fracture porosity$\phi_{F}$      & $0.2$\\
 \hline
\end{tabular}
\label{tab:param_3}
\end{table}



\begin{figure}[hbt!]
\centering
\includegraphics[width=10cm]{figures_new/small_features/small_feat_geo}
\caption{Geometry Setup and Boundary Conditions (top). Fracture Network (Bottom).}
\label{fig:small_feat_p_1_2_res}
\end{figure}



\begin{figure}
\centering
\subfloat[Unresolved case 1]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea1grid.png}}
\subfloat[Unresolved case 2]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea2grid.png}}\\
\subfloat[Unresolved case 3]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea4grid.png}}
\subfloat[Unresolved case 4]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea6grid.png}}
\label{mesh_unreolved}
\end{figure}

\begin{table}[ht]
\caption{Mesh Setting}
\centering
\begin{tabular}{ |p{2cm}||p{2cm}|p{2cm}|p{2cm}|  }
 \hline
 \multicolumn{4}{|c|}{Resolved Mesh} \\
 \hline
          &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# layers\\
 \hline
$\mathrm{res_1}$    &     3823   &     19964 & 1\\ 
$\mathrm{res_2}$    &      28519   &     159712  & 2\\
$\mathrm{res_3}$    &      220325   &    1277696  &  3\\
$\mathrm{res_4}$    &   1732172   &    10221568 &  4\\
 \hline
 \multicolumn{4}{|c|}{Unresolved Mesh} \\
  \hline
          &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# layers\\
 \hline
$\mathrm{unres_1}$    &      667672  &      560290 & ~1\\ 
$\mathrm{unres_2}$    &           964549   &      933120  & ~2\\
$\mathrm{unres_3}$    &     18634058   &    16727570  &  ~3\\
$\mathrm{unres_4}$    &     90026102  &     84703700 &  ~6\\
 \hline
\end{tabular}
\label{tab:mesh_3}
\end{table}

\subsection{Small Features}
%\begin{enumerate}
%\item  we observe a slow convergence for both the resolved and the unresolved case. Jump in the values used for the constitutive parameters and  for the neumann boundary conditions  affect the regularity of the solution and (The regularity of  the solution is less than $H^2$). A priori, both these issues reduce the convergence rate of the FE method, as the sol must be at least $p-1$ in order to converge with order $p$. The reduction of the convergence rate  due to the jump in the parameters can be avoided with a mesh that resolves the boundary of the discontinuity. In this case, we may get the expected order of convergence. Instead, the problem related to the  discontinuities in the values used for the boundary conditions can not be avoided in any way with the standard continuous fe methods. Possible solutions are to use methods GFEM or multiscale that add special functions to the type of discontinuity, or try to make AMR near the region where boundary conditions changes occur. (Maybe we can mention this also for the regular case)
%\item for the plots over region one may notice a good agreement between the resolved and the unresolved case. Can we say the same also for the pressure?
%\end{enumerate}

\begin{figure}
\centering
\subfloat[a)Spatial  distribution of the pressure]{\includegraphics[width=10cm]{figures_new/small_features/p_small_feat_1}}\\
\subfloat[b) Spatial  distribution of the pressure in the planes $x=0.5$ and $z=0.5$ where line $A-A^{\prime}$ and $B-B^{\prime}$ lie]{\includegraphics[width=10cm]{figures_new/small_features/p_small_feat_2}}
\label{fig:small_feat_p_unres}
\end{figure}




\begin{figure}
\centering
\includegraphics[width=6cm]{figures_new/small_features/resolved/fig_1}
\includegraphics[width=6cm]{figures_new/small_features/resolved/fig_2}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_p_1_2_res}
\end{figure}


\begin{figure}[hbt!]
\centering
\includegraphics[width=6cm]{figures_new/small_features/unresolved/fig_1}
\includegraphics[width=6cm]{figures_new/small_features/unresolved/fig_2}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_p_1_2_unres}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=6cm]{figures_new/small_features/fig_1}
\includegraphics[width=6cm]{figures_new/small_features/fig_2}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_comp}
\end{figure}
\begin{figure}[hbt!]
\hspace{-0.8cm}\includegraphics[width=14cm]{figures_new/small_features/fig_3}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_conc}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=8cm]{figures_new/small_features/c_small_feat}
\caption{Concentration at last time step.}
\label{fig:small_feat_c_ures}
\end{figure}




This benchmark allows for testing the accuracy of the proposed method in the presence of small geometric features. The matrix background is a box $M=(0\,;\,1)\times(0\,;\,2.25)\times(0\,;\,1)\, m$, containing eight fractures.
These are defined by their vertexes and described in~\cite{flemisch2018benchmarks}. The inlet and the outlet are defined as follows: $\partial \Omega_{in}=(0\,;\,1)\times(0)\times(1/3\,;\,2/3)\,m$, $\partial \Omega_{out,1}=(0\,;\,1)\times(2.25)\times(0\,;\,1/3)\,m$,
$\partial \Omega_{out,2}=(0\,;\,1)\times(2.25)\times(1/3\,;\,2/3)\,m$. 

For the flow problem, a uniform inflow on the inlet such that $\int_{\partial \Omega_{in}}\mathbf{u}\cdot \mathbf{n}\,d\gamma=-1/3$, whereas homogeneous Dirichlet boundary conditions are applied on the outlet $\partial \Omega_{out}=\partial \Omega_{out,1}\cup\partial \Omega_{out,2}$. No flow (Neumann) boundary conditions are set on the other boundaries. 

For the transport problem, a Dirichlet boundary condition is imposed on the inlet: $c_{in}=1.0\,m$.
The overall simulation time is set equal to $t_f=10^{2}\,s$ while the time step is set equal to$dt=0.01$.  All the material parameters are summarized in table~\ref{tab:param_3}:


Table ~\ref{tab:mesh_1} lists the number nodes and elements for all performed test cases. As an example, in Figures \ref{mesh_unreolved} and ~\ref{p_small_feat_2} we show the meshes obtained by adopting the adaptive refinement to model the fracture network geometry for all the unresolved test cases reported in Table ~\ref{tab:mesh_1}, and the spatial distribution obtained for test case $\rm{unres}_3$ . In particular ~\ref{p_small_feat_2} b) depicts the spatial distribution of the pressure at planes $x=0.5$ and $z=0.5$ and the extreme points $A=(0.5,\,1.1,\,0)-A^{\prime}=(0.5,\,1.1,\,1)$, and $B=(0,\,2.15,\,0.5)-B^{\prime}=(1,\,2.15,\,0.5)$ of the lines along which the pressure profiles are analized.

Figures~\ref{fig:small_feat_p_1_2_res} and ~\ref{fig:small_feat_p_1_2_unres} depict the pressure profile along the line $A-A^{\prime}$ and $B-B^{\prime}$, for the resolved and the unresolved test cases reported in Table~\ref{tab:mesh_3}. 
We observe that the accuracy of the solution strongly depends on the mesh size for all the performed numerical simulations. 
Figure~\ref{fig:small_feat_comp} shows a comparison between the test cases $\rm{res_4}$ and $\rm{ures_4}$. Small discrepancies can be appreciated since mesh converge was observed neither for the unresolved nor for the resolved test case.

In this regard, it is worth mentioning that the jumps in the values used for the constitutive parameters and the Neumann boundary conditions affect the regularity of the solution. A priori, both these issues reduce the convergence rate of the FE method, as the sol must be at least $p-1$ to converge with order $p$. The reduction of the convergence rate due to the jump in the parameters can be avoided with a mesh that resolves the boundary of the discontinuity. In this case, we may get the expected order of convergence. Instead, the problem related to the discontinuities in the values used for the boundary conditions can not be avoided in any way with the standard continuous Finite Element  Methods. Possible solutions are to use methods GFEM or multiscale that add special functions to the type of discontinuity or try to make AMR near the region where boundary conditions changes occur.
Finally, we analyze the average concentration in each fracture and plot the results in Figure~\ref{fig:small_feat_conc} which reveals a good agreement between the test cases $\rm{res_4}$ and $\rm{ures_4}$. Indeed, as one may observe
figures~\ref{fig:small_feat_p_1_2_res} and ~\ref{fig:small_feat_p_1_2_unres}, the progressive refinement performed to solve for the flow problem, produces as the main effect the sum of a constant to the coarsest solution. Hence, even though the values of the pressure field increase,  the computation of the corresponding gradient, and consequently of the velocity field, will produce similar results.







\subsection{Hydrocoin}
%\begin{enumerate}
%\item good agreement between unresolved and the reference solution
%\end{enumerate}
This flow problem was presented within the international Hydrocoin project, (Swedish Nuclear Power Inspectorate (SKI) and proposed as benchmark for both hybrid and equi-dimensional models in~\cite{flemisch2018benchmarks}. Concerning the boundary conditions,  a piezometric head is imposed on the top boundary of the domain, whereas  no  flow (Neumann) boundary conditions are set on the other boundaries. We only consider the unresolved test case consisting of $12683$ elements and $10938$ nodes and compare the corresponding solution for the pressure with the reference  solution obtained by a standard FV method on a continuous fracture model and computed on a grid with $3 527 296$
elements and $3 813 249$ nodes ~\cite{flemisch2018benchmarks}. 
\begin{table}[htb!]
\caption{Parameters Setting for conductivity and porosity}
\centering
\begin{tabular}{ |p{4cm}||p{1cm}|}
 \hline
 \multicolumn{2}{|c|}{Parameters Values} \\
 \hline
matrix conductivity $K_{M}$    &  $10^{-8}$ \\
fracture conductivity $K_{F}$    &  $10^{-6}$ \\
 \hline
\end{tabular}
\label{tab:param_1}
\end{table}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm ]{figures_new/hydro}
\caption{Benchmark 1. Locally refined mesh with Ndof equato to 259600 (AMR$_5$). Fractures are represent by means an AME techniques,}
\label{fig:setup_hydro}
\end{figure}
\begin{figure}[ht]
\centering
\includegraphics[width=7cm]{figures_new/hydrocoin/fig}
\caption{Pressure profiles for  the benchmark \textit{hydrocoin} along the line $A-A^{\prime}$ }
\label{fig:hydro_p}
\end{figure}


Figure~\ref{fig:setup_hydro} shows the pressure distribution and the extreme points of  $A=(0\,;\,-200\,;\,0)$ and $A^{\prime}=(1600\,;\,-200\,;\,0)$ of the line along which the pressure is analyzed.  In Figure~\ref{fig:hydro_p}, we observe a good agreement between the numerical results obtained for the unresolved test case and the reference solution.


\subsection{Realistic}

In this last test case, we consider a real set of fractures from an interpreted outcrop in the Sotra island, near Bergen in Norway. The set comprises
64 fractures grouped in 13 different connected networks, ranging from isolated fractures up to tens of fractures each. In the interpretation process, two fractures are composed of more than one segment. The size of the domain is $700\,m \times 600 \,m$ with uniform matrix permeability $K_m = 10$. For simplicity, all the fractures have the same scalar permeability $K_f=10^{-6}$. Concerning the boundary conditions, we consider homogeneous Neumann boundary conditions (no flow) on the top and bottom side, a pressure $P= 1013250\,[Pa]$ is applied on the left side, and pressure $P=0\,[Pa]$ on the right side of the domain.
In Figure~\ref{fig:realistic_line_1} we analize the mesh converge by analyze the pressure along the lines $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for all the unresolved test cases reported in Table~\textbf{add table}.
While we observe that all the pressure profiles show similar behavior, relevant differences are found in the pressure distribution reported in Figure~\ref{fig:realistic_pressure} where a similar pattern is only observed for the test cases $\rm{unres_3}$ and $\rm{unres_4}$.
Figure~\ref{fig:realistic_line_1} shows a comparison between our numerical results and those obtained with the numerical methods presented in ~\cite{flemisch2018benchmarks}. Again a good agreement is found among all the profiles. 

\begin{figure}
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh0.pdf}}
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh3.pdf}}\\
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh4.pdf}}
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh6.pdf}}
\end{figure}



\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm]{figures_new/realistic/convergence}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:realistic_line_1}
\end{figure}



\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{figures_new/realistic/fig_realistic_p_tot}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:realistic_pressure}
\end{figure}


\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm]{figures_new/realistic/comparison}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:realistic_line_1}

\end{figure}



\newpage

%\printbibliography





==> sections/06ResultsSave.tex <==
\section{Numerical examples}

In this section, we validate the proposed approach using five benchmark cases. The first benchmark is s a two-dimensional version of the test case proposed in~\cite{BenchPaper}
The second benchmark case is based on Geiger et al. (2013) ~\cite{flemisch2018benchmarks} and shows a regular fracture network. The third test case is based on a well-established benchmark for groundwater flow from Swedish Nuclear Power Inspectorate (SKI) (1987). The fourth taste case is a three-dimensional test case containing small geometric features~\cite{BenchPaper}, whereas the last benchmark considers a realistic scenario where several fractures randomly oriented are embedded in a rock matrix.

For each benchmark,  we consider both the resolved and the unresolved test cases and compare the numerical results in terms of pressure and concentration profiles along the prescribed lines.


\subsection{Adaptive mesh refinement\\ for heterogenous media}

In this section, we briefly summarize the AMR method, whose details are presented in \cite{Holliger2000}.
The idea at the base is to start with a coarse uniform mesh.
In particular, for cuboid domains of tipe $\Omega^c$,
the initial mesh can also be thought as structured.
The initial mesh is not supposed to explicitly resolved the interfaces between the background and the fractures.

Then, given a distribution of embedded fractures,
we iterate over all elements and mark for refinement the ones that have non-empty intersections with the boundary of at least one fracture.

In some cases, it can be useful to change the target according to which we decide to mark for refinement.
For example, when conductive fractures are considered, i.e., fractures which have a permeability much larger compared to the one of the matrix,
it is convenient to mark for refinement all the elements that have a non-empty overlap with at least one fracture.
This means that elements insides a fracture are refined as well.
Moreover, the refinement region can be a region around the fracture but not necessarily coinciding with the fracture.


This procedure allows to create a sequence of meshes, which become progressively finer towards the interfaces.
This AMR method allows to automatically create meshes for any heterogeneity distribution without any human interaction.
In order to keep the meshes $1$-irregular, at each step the refinement region may be enlarged in order to satisfy such a constraint.


%In order to evaluate the accuracy of the method, solutions or output variables, such as seismic attenuation and velocity dispersion,
%from two consecutive hierarchical levels can be compared.

%Another possibility for evaluating the quality of the solution would be to employ error estimators,
%which are not readily available for the proposed method.
%In this regard, there are basically two options.
%One would be to adapt error estimators based on flux reconstruction that have already been developed for Biot's equations in the time domain \cite{RIEDLBECK20171593}.
%Here, the main difficulty would be to extend this methodology to complex vector spaces and non-symmetric problems.
%Another would be to use more generic residual-based error estimators for coupled problems, e.g. \cite{ern2009posteriori}.


\subsection*{Resolved and unresolved discretizations}
We finally introduce two different methods to simulate flow and transport in fractured media.

\textit{Resolved discretization} The first discretization will be referred to as \emph{resolved} and its meshes resolve the interfaces between the matrix and the fractures. It makes use of conforming meshes which are, in general, complicated to generate,
since they require a lot of human-computer interaction to achieve the desired mesh quality. The mesh generation of a fractured network system is usually tedious and difficult  to make automatic due to the geometric complexity of the computational domain induced by existence and extension of fractures.

\textit{Unresolved discretization} The second discretization will be referred to as \emph{unresolved} and its meshes do not explicitly resolve the interfaces between the matrix and the fractures,
but are actually refined close to such interfaces. More specifically an adaptive refinement procedure is adopted to ensure the desired leyer of elements inside  each fracture network. Given a mesh $\mathcal{T}$, each element is initially marked as belonging to either the background matrix or to the fracture network. Then all the elements marked as \textit{fractured} are progressively refined until the desired mesh-accuracy is achieved.

\textbf{Remark} For the unresolved discretization, all the bilinear and linear operators, i.e matrices and vectors, are computed element-wise on the non-conforming space $W^H$ and them projected onto the regular space $V^r$ by means of the interpolation operator~\eqref{eq:interp}.

It is worth to pointing out that, the stabilization of the transport problem can be also either performed on the  transport operator $\mathbf{A}$ or on its element-wise contribution $[\mathbf{A}]_{ij}$ . While there is no difference between the two approaches when conforming meshes are adopted, the use of non-conforming meshes makes mandatory the first approach. Indeed, if one stabilize the local contribution $[\mathbf{A}]_{ij}$, the subsequent use of the relation $\eqref{eq:intA}$ introduces off diagonal entries which violate the assumptions 1a and 1b of theorem~\ref{th:DM} needed to ensure the DMP.

According to the definitions above, a triangulation can be non-conforming and non-uniform but all elements are shape-regular, being squares or cubes.



%\textbf{It is also a very tedious task to create a full-dimensional description of the fracture network and a corresponding equi-dimensional grid of the whole computational domain. Therefore, we refrain from calculating a reference solution with the MFD method and per- form a direct comparison of the hybrid-dimensional methods.
%It is also a very tedious task to create a full-dimensional description of the fracture network and a corresponding equi-dimen- sional grid of the whole computational domain. Therefore, we refrain from calculating a reference solution with the MFD method and per- form a direct comparison of the hybrid-dimensional methods..}

%Ciò che inficia la regolarità sono i jump nei parametri (mi sembra che la sol appartenga a H^5/4) e particolari cambi di boundary conditions (La sol è meno di H^2). A priori entrambi questi problemi riducono la convergenza dei metodi fe, in quanto la sol deve essere almeno in p+1 al fine di avere convergenza con ordine p. Il converence rate ridotto dovuto ai jump nei parametri può essere evitato con mesh che risolvono i boundary delle discontinuità. In questo caso si ottengono ordini di convergenza simili al problema senza discontinuità, con il fatto che se ci sono molte discontinuità sono difficili da meshare. Invece il problema legato alla discontinuità del tipo di boundary conditions non può essere evitato in alcun modo con i fe standard. Possibili soluzioni sono usare metodi GFEM o multiscala che aggiungono particolari funzioni legate al tipo di discontinuità oppure provare a fare AMR vicino al cambio del tipo di boundary conditions.}


\subsection{Single 2D}
%\begin{enumerate}
%\item good agreement between unresolved and resolved
%\item for the resolved case meshes comprising poor-quality elements may affect the accuracy of the method as shown in Figure~2
%\end{enumerate}
The first benchmark example consists of a square-shaped domain $\Omega_{M}$ crossed by a an oblique fracture $\Omega_{F}$ with a thickness $\delta=0.01$. To represent an heterogeneous rock matrix, different material properties are assigned to a sub-domain $\Omega_{het}$ defined in lower part of the domain $M$.  A geometrical description of the rock matrix and the fracture are depicted in Figure, whereas more details on the geometrical sizes can be found in Table~\ref{tab:geo_1}.
\begin{table}[ht]
\caption{Geometrical sizes}
\centering
\begin{tabular}{ |p{1cm}||p{1cm}|p{1cm}|p{1cm}| |p{1cm}|  }
 \hline
 \multicolumn{5}{|c|}{Rock Matrix} \\
 \hline
      & {$\bf{x_{s}}$} [m]& $\bf{x_{e}}$ [m]& $\bf y_{s}$ [m]& $\bf y_{e}$ [m] \\
 \hline
$\mathrm\Omega_{M}$ &-50 & 50 & -50 & 50    \\
$\mathrm\Omega_{het}$  &-50 & 50 & -50 & -40  \\
$\mathrm{\Gamma_{in}}$  &0 & 0 & 40 & 50  \\
$\mathrm{\Gamma_{out}}$  &50 & 50 & 0 & 10  \\
 \hline
 \multicolumn{5}{|c|}{Fracture} \\
  \hline
      & $ \bf x_{s}$ [m]& $\bf x_{e}$ [m]& $\bf y_{s}$ [m]& $\bf y_{e}$ [m]  \\
 \hline
 $\mathrm\Omega_{F}$& -50   & 50 & -30 & 30\\
 \hline
\end{tabular}
\label{tab:geo_1}
\end{table}

Concerning the boundary conditions, for the flow problem, we impose a Dirichlet condition at the inlet $\Gamma_in$ with $p_{in}^{D}= 4m$ and at the outlet $\Gamma_{out}$ with $p_{out}^{D} = 1m$,  whereas for the transport problem, we impose a Dirichlet condition $c_{in}^{D} = 0.01m^{2}$ at the inlet $\Gamma_{in}$.  For the transport problem, the overall simulation time is $t_f=10^{9}\,\rm{[s]}$ and the time step is $dt=10^2~\rm{[s]}$. The parameters adopted for the material properties are summarized in Table~\ref{tab:geo_1}. 


\begin{table}[ht]
\caption{Parameters Setting for conductivity and porosity}
\centering
\begin{tabular}{ |p{4cm}||p{1cm}|}
 \hline
 \multicolumn{2}{|c|}{Parameters Values} \\
 \hline
matrix conductivity $\bf K_{M1}$    &  $10^{-6}$ \\
matrix conductivity $\bf K_{M2}$    &  $10^{-5}$ \\
fracture conductivity $\bf K_{F}$     &   $10^{-1}$ \\
matrix porosity$\boldsymbol{\phi_{M1}}$    & $0.2 $ \\
matrix porosity $\boldsymbol{\phi_{M2}}$   & $0.2$  \\
matrix porosity $\boldsymbol{\phi_{M3}}$   &  $0.25$ \\
fracture porosity$\boldsymbol{\phi_{F}}$      & $0.4$\\
 \hline
\end{tabular}
\label{tab:param_1}
\end{table}

Four different meshes are considered for the resolved and the unresolved configurations. In Table~\ref{tab:mesh_1} we report the number of nodes, elements and layer of elements inside the fracture for each test case. 
\begin{figure}[hbt!]
\centering
\includegraphics[width=9cm]{figures_new/single/fig_mesh_unres}
\caption{Locally refined mesh for the test case $\rm{unres_3}$. }
\label{fig:single_unresolved_mesh}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm ]{figures_new/single_p}
\caption{Pressure distribution for the test case $\rm{unres_3}$ (Units [Pa]).}
\label{fig:single_p_unresolved_setup}
\end{figure}

%\begin{figure}[hbt!]
%\centering
%\hspace{0.1cm}
%\includegraphics[width=11cm ]{figures_new/single/single_c_tot}
%\caption{Concentration distribution at time $t=2\,10^{8}[s]$ and $t=\,10^{9}[s]$ for the test case $\rm{unres_3}$ (Units [m]).}
%\label{fig:unresolved_single_c}
%\end{figure}

As an example, in Figures~\ref{fig:single_unresolved_mesh}, \ref{fig:single_p_unresolved_setup} and~\ref{fig:unresolved_single_c} we show  the mesh used for the test case $\mathrm{unres_3}$,   the corresponding solution obtained by solving the flow problem, and  the one resulting from the transport problem, respectively. In particular, we in Figure~\ref{fig:unresolved_single_c} we show the concentration distribution at the time instants $t=2\,10^{8}[s]$ and $t=\,10^{9}[s]$.  The obtained results confirm the ability of  stabilization technique to preserve the positivity of the solution and ensure the local maximum principle.


\begin{table}[ht]
\caption{Mesh Setting for Benchmark Single 2D}
\centering
\begin{tabular}{ |p{2cm}|p{2cm}|p{2cm}|p{1cm}|p{2cm}|p{2cm}|  }
 \hline
 \multicolumn{6}{|c|}{Resolved Mesh} \\
 \hline
      &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
$\mathrm{res_1}$&\,\,\,\,\,\,\,6\,785  &\,\,\,\,\,\,\,6\,612 &  1& $1.86675\,e^{-6}$  & $-1.86675\,e^{-6}$\\
$\mathrm{res_2}$&\,\,\,26\,793  &\,\,\,\,26\,448 &  2& $1.85977\,e^{-6}$  & $-1.85977\,e^{-6}$\\
$\mathrm{res_3}$& 106\,481  & 105\,792 &  3& $1.85632\,e^{-6}$  & $-1.85632\,e^{-6}$\\
$\mathrm{res_4}$& 424\,545  & 423\,168 &  4& $1.85457\,e^{-6}$  & $-1.85457\,e^{-6}$\\
 \hline
 \multicolumn{6}{|c|}{Unresolved Mesh} \\
  \hline
        &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
 $\mathrm{unres_1}$&\,\,\,\,162\,628   &\,\,\,\,141\,640  & 1.28  & $1.86277\,e^{-6}$ & $-1.86277\,e^{-6}$\\
  $\mathrm{unres_2}$&\,\,\,\,401\,680   &\,\,\,\,442\,813  & 2.56  & $1.85779\,e^{-6}$ & $-1.85779\,e^{-6}$\\
 $\mathrm{unres _3}$&1\,291\,360      &1\,375\,252 & 5.12       &$1.85534\,e^{-6}$ & $-1.85534\,e^{-6}$ \\
 $\mathrm{unres _4}$&2\,678\,304      &2\,512\,480 &10.24      & $1.85517\,e^{-6}$ & $-1.85517\,e^{-6}$ \\
 \hline
\end{tabular}
\label{tab:mesh_1}
\end{table}




\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/single/conservation}
\caption{Flux conservation}
\label{fig:single_flux}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/single/pressure}
\caption{Pressure Profile}
\label{fig:single_P}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/single/concentration}
\caption{Concentration}
\label{fig:single_CM}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=8cm]{figures_new/single/fig_mesh_res}
\caption{Left: mesh of the test case $\rm{res_{1,\rm{uni}}}$ together with a zoom-in of the region close to end point $\rm B^{\prime}$. Right: comparison between  the concentration profiled obtained for the test cases $\rm{res_{1,\rm{uni}}}$  and  $\rm{res_1}$ along the line $\rm{B-B^{\prime}}$.}
\label{fig:mesh_c_recolved_bench_1}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/single/concentration_correction_2}
\caption{Concentration distribution at time $t=2\,10^{8}[s]$ and $t=\,10^{9}[s]$ for the test case $\rm{unres_3}$ (Units [m]).}
\label{fig:unresolved_single_c}
\end{figure}

%\begin{figure}[hbt!]
%\includegraphics[width=6cm]{figures_new/single/resolved/fig_1}
%\includegraphics[width=6cm]{figures_new/single/unresolved/fig_1}
%\caption{Pressure profiles along the line $\rm{A-A^{\prime}}$ for all the resolved (left) and unresolved (right) cases presented in Table~\ref{tab:mesh_1}. }
%\label{fig:figure_p_res_unres_bench1}
%\end{figure}
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=7cm]{figures_new/single/fig_1}
%\caption{Pressure profiles along the line $\rm{A-A^{\prime}}$ for the finest resolved and unresolved test cases, respectively.}
%\label{fig:figure_p_comp_bench1}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/single/resolved/fig_2}
%\includegraphics[width=6cm]{figures_new/single/unresolved/fig_2}
%\caption{Concentration profiles  at final time along the line $\rm{A-A^{\prime}}$ for all the resolved (left) and unresolved (right) cases presented in Table~\ref{tab:mesh_1}. }
%\label{fig:figure_c1_bench1}
%\end{figure}


%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/single/resolved/fig_3}
%\includegraphics[width=6cm]{figures_new/single/unresolved/fig_3}
%\caption{Concentration profiles  at final time along the line $\rm{B-B^{\prime}}$ for all the resolved (left) and unresolved (right) cases presented in Table~\ref{tab:mesh_1}.}
%\label{fig:figure_c2_bench1}
%\end{figure}
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/single/fig_3}
%\includegraphics[width=6cm]{figures_new/single/fig_2}
%\caption{Concentration profiles  at time $t=t_f$ along the line $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for the finest resolved and the unresolved test case, respectively.}
%\label{fig:figure_c_comp_bench1}
%\end{figure}







We validate our approach by analyzing the pressure and the concentration profiles along the lines connecting the points $\rm{A-A^{\prime}}$, with coordinates $\rm{A}=(50;-50;0)$, and $\rm{A^{\prime}}=(-50;50;0))$, and $\rm{B-B^{\prime}}$, with coordinates $\rm{B}=(30;-30;0)$, and $\rm{B^{\prime}}=(-30;30;0))$, as depicted in Figure~\ref{fig:single_p_unresolved_setup}.

In Figures~\ref{fig:figure_p_res_unres_bench1} and~\ref{fig:figure_p_comp_bench1} we compare the pressure computed along the line $\rm{A-A^{\prime}}$ for all the test cases presented in Table~\ref{tab:mesh_1}. No relevant differences are found among all the numerical results (Figure~\ref{fig:figure_p_res_unres_bench1}) and a good agreement is observed between the resolved and the unresolved solution (Figure~\ref{fig:figure_p_comp_bench1}).


In Figures~\ref{fig:figure_c1_bench1} and ~\ref{fig:figure_c2_bench1} the concentration obtained at time $t=t_f$ along the lines $\rm{A-A^{\prime}}$ and  $\rm{B-B^{\prime}}$ is plotted. Again, all the analyzed profiles reveal a similar behaviour and a good match is found between the resolved and the unresolved results, as shown in Figure~\ref{fig:figure_c_comp_bench1}.

It is worth pointing out that the use of adaptive refinement allows controlling the quality of the mesh which represents an important requirement to ensure the stability of the method and accuracy of the solution. In this regard, in Figure~\ref{fig:mesh_c_recolved_bench_1} we show a comparison between the concentration obtained for the test cases $\rm{res_{1,\rm{uni}}}$ and $\rm{res_1}$ along the line $\rm{B-B^{\prime}}$. Differences can be clearly observed close to the endpoint $\rm{B^{\prime}}$ and are mainly related to the poor-quality of the mesh $\rm{res_{1,\rm{uni}}}$ obtained by performing one uniform refinement step on the mesh used for the test case $\rm{res_{1}}$.




\subsection{Regular}
%\begin{enumerate}
%\item good agreement between unresolved and resolved
%\item for the unresolved we observe a deviation the solution along line 2 whereas along line 1 (fracture in the middle) we get good match for both the resolved the unresolved meshes.
%Can we justify the deviation with the low order of convergence due to the discontinuity in both parameters and boundary conditions? this hypothesis seems to be supported from the fact that in the blocking case we get good agreement with respect to the reference solution for both resolved and the unresolved mesh. 
%\item for the concentration can we justify the differences between the resolved and the unresolved case in the same way as done for the pressure?
%\item for the plots over region the concentration seems to tend to zero in regions 2 4 and 6 (figure 18). The diffusion added by the stabilization term seems to prevent the solution to go to zero (shell we mention this?). Can  we refer to the  differences between the solutions in these regions to justify also the differences obtained in the plots over line (see figures~15 and 17)?
%\end{enumerate}

The second benchmark consists of a regular fracture network embedded in square with size $x_s=0\,m\,x_e=1\,m$ and $y_s=0\,m\,y_e=1\,m$. The rock has a unitary conductivity $K_M = I$, whereas for the fractures we consider two cases: a highly conductive fracture network with $K_F = 10^4$ and a blocking fracture network with $K_F=10^{-4}$. For the transport problem, the matrix and the fracture network have the same porosity,~i.e. $\phi_m=\phi_f=1.0$.

For the flow problem, we apply homogeneous Neumann conditions (no flow) on top and bottom sides, a unitary inflow flux $u_N=-1$ on the left boundary, and a Dirichlet condition $p_D = 1$ on the right boundary. Our numerical results are compared with the numerical approaches and the reference solution presented in~\cite{flemisch2018benchmarks}. 

For the transport problem, a unitary concentration $c_d=1.0$ is imposed on the left boundary, whereas homogeneous Neumann conditions (no flow) are applied on the remaining sides.  The time step $dt=0.025~\rm{[s]}$ and the overall simulation time is set equal to$t_f=0.5,~\rm{[s]}$. 





%    \begin{figure}[hbt!]
%    \centering
%    \includegraphics[width=3.8cm]{figures/regular/RegularConfC1.eps}
%    \includegraphics[width=3.8cm]{figures/regular/RegularAMRC1.eps}
%    \includegraphics[width=3.8cm]{figures/regular/RegularConfAMRC1.eps}
%    \caption{Benchmark 2 with conductive fractures: comparison of concentration values along the line $y=0.5$}
%    \label{fig:figure_p1_bench2}
%    \end{figure}

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=3.8cm]{figures/regular/REgularConfC2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularAMRC2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularConfAMRC2.eps}
%\caption{Benchmark 2 with conductive fractures: comparison of concentration values along the line $y=0.5$}
%\label{fig:figure_p1_bench2}
%\end{figure}

% \begin{figure}[hbt!]
% \centering
% \includegraphics[width=8cm]{figures/RegularVerticalLine}
% \caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $x=0.5$.}
% \label{fig:figure_p2_bench2}
% \end{figure}




\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm]{figures_new/regular_p}
\caption{Pressure distribution for the test case $\rm{unres_3}$ (Units [Pa])}
\label{fig:unresolved_regular_p}
\end{figure}


%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=10cm]{figures_new/regular_c_tot}
%\caption{Concentration distribution at time $t=\,0.20[s]$ and $t=\,0.5[s]$ for the test case $\rm{unres_3}$ (Units [m]).}
%\label{fig:unresolved_regular_c}
%\end{figure}

\subsubsection{Conductive fracture network}
First, we consider a highly conductivity network. Three different meshes are considered for the resolved and the unresolved configurations. In Table ~\ref{tab:mesh_2} we report the number of nodes, elements and layer of elements inside the fracture for each test case.

\begin{table}[ht]
\caption{Mesh Setting for Benchmark Regular 2D}
\centering
\begin{tabular}{ |p{2cm}|p{2cm}|p{2cm}|p{1cm}|p{2cm}|p{2cm}|  }
 \hline
 \multicolumn{6}{|c|}{Resolved Mesh} \\
 \hline
      &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
%$\mathrm{unres_0}$&     29929 &   29584    &  4\\
$\mathrm{unres_1}$&   110889 &  110224    &  4&  0.662191 & -0.662191\\
$\mathrm{unres_2}$&   426409 &  425104   &  4 & 0.662189 & -0.662189\\
$\mathrm{unres_3}$&   1671849    & 1669264   &  4 & 0.662185&-0.662185\\
$\mathrm{unres_4}$&    16056049   &   16048036  &  2&  0.662177 & -0.662177\\
 \hline
 \multicolumn{6}{|c|}{Unresolved Mesh} \\
  \hline
      &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# l& flux$_{1}$ & flux$_{2}$\\
 \hline
$\mathrm{unres_1}$&  1\,863\,685 &    1\,720\,768    &  4& 0.65692& -0.65692\\
$\mathrm{unres_2}$&     1\,879\,729 &   1\,736\,896  &  4 &0.656915 &-0.656915 \\
$\mathrm{unres_3}$&    4\,673\,031     &  4\,387\,096   &  8 &0.662382 &-0.662382\\
$\mathrm{unres_4}$&      4\,966\,635   &  4\,681\,144   &  8& 0.662381& -0.662381\\
$\mathrm{unres_5}$&        15\,054\,349   &    14\,483\,152   &  16&0.662415&-0.662415\\
 \hline
\end{tabular}
\label{tab:mesh_2}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c| c |}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11\\
80 &  &  &  &  &  &  0.12045&  0.11707&  0.11704&  0.11823&  0.1182 \\
160 &  &  &  &  &  0.12031&  0.11692&  0.11691&  0.11811&  0.11808&   \\
320 &  &  &  &  0.12023&  0.11684&  0.11683&  0.11803&  0.11801&  &   \\
640 &  &  &  0.1202&  0.11679&  0.11679&  0.11799&  0.11797&  &  &   \\
1280 &  &  0.12018&  0.11677&  0.11677&  0.11797&  0.11794&  &  &  &   \\
2560 &  0.12017&  0.11676&  0.11676&  0.11796&  0.11793&  &  &  &  &   \\
\end{tabular}
\caption{flussi unresolved stab}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c| c |}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 \\
80 &  &  &  &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11776 \\
160 &  &  &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&   \\
320 &  &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &   \\
640 &  &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &  &   \\
1280 &  &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &  &  &   \\
2560 &  0.11677&  0.11675&  0.11675&  0.11778&  0.11777&  &  &  &  &   \\
\end{tabular}
\caption{flussi unresolved non-stab}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c| c |}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 \\
80 &  &  &  &  &  &  474.29&  951.49&  3537.8&  9321.43&  30687.04 \\
160 &  &  &  &  &  533.79&  997.24&  3541.53&  9293.61&  29055.21&   \\
320 &  &  &  &  825.26&  1305.83&  3817.38&  9345.93&  28419.23&  &   \\
640 &  &  &  1573.17&  2161.3&  4909.56&  10994.99&  29168.34&  &  &   \\
1280 &  &  5397.39&  6343.81&  9328.68&  15453.4&  37212.82&  &  &  &   \\
2560 &  10726.8&  11474.12&  13512.52&  17933.18&  31340.79&  &  &  &  &   \\
\end{tabular}
\caption{solution time non stab, decidi se torna utile}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | }
 & 1 & 2 & 4 & 8 & 16 \\
80 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11775 \\
160 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11775 \\
320 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11775 \\
640 &  0.11775&  0.11775&  0.11775&  0.11775&  0.11776 \\
1280 &  0.11775&  0.11775&  0.11776&  0.11776&  0.11776 \\
\end{tabular}
\caption{flussi resolved}
\end{table}

\begin{table}[ht]
\begin{tabular}{| c | c | c | c | c | c | }
 & 1 & 2 & 4 & 8 & 16 \\
80 &  44.03&  43.74&  44.56&  33.11&  42.12 \\
160 &  59.9&  67.31&  70.1&  76.72&  96.27 \\
320 &  216.14&  212.6&  220.18&  220.88&  259.91 \\
640 &  844.39&  816.7&  918.61&  888.23&  1007.48 \\
1280 &  3678.56&  3725.55&  3476.15&  3829.14&  3680.57 \\
\end{tabular}
\caption{solution time resolved, direi che non \'e utile}
\end{table}

In Figure~\ref{fig:unresolved_regular_p} we show the spatial distribution of the pressure, and  the extreme points of the lines $A-A^{\prime}$, $(x=0.5)$, and $B-B^{\prime}$, $(y=0.75)$ along which we perform our analysis.
Figures~\ref{fig:regular_p1_res_unres} and ~\ref{fig:regular_p1_res_unres} depict the pressure profile along the line $A-A^{\prime}$ and  $B-B^{\prime}$,  for the resolved and the unresolved test cases reported in Table~\ref{tab:mesh_2}. Here, one may observe that all the solutions exhibit a similar behaviour. Figure~\ref{fig:regular_p1_p2_comp} shows a comparison with the numerical methods and the reference solution presented in ~\cite{flemisch2018benchmarks}. It refers to a very fine reference mesh, with a total of $1\,175\,056$ element, where the fractures are resolved by ten elements in their normal direction.

While all the results reveal a good match for line $A-A^{\prime}$, a small deviation is found for the test case $\rm{unres_3}$ along the line $B-B^{\prime}$, where our method shows a good agreement with the Embedded Discrete Fracture Method (EDFM).
\begin{table}[ht]
\caption{List of Regions}
\centering
\begin{tabular}{ |p{2cm}||p{2cm}|p{2cm}|  }
 \hline
      & $\mathbf{x}_{range}$    & $\mathbf{y}_{range}$ \\
       \hline
$\mathrm{1}$&  [0\,\,0.5] &   [0\,\,0.5]   \\
$\mathrm{2}$&   [0.5\,\,1.0] &   [0\,\,0.5]   \\
$\mathrm{3}$&  [0\,\,0.5]     &  [0.5\,\,1.0]    \\
$\mathrm{4}$&  [0.75\,\,1.0]     &  [0.75\,\,1.0]    \\
$\mathrm{5}$&  [0.75\,\,1.0]     &  [0.5\,\,0.75]    \\
$\mathrm{6}$&  [0.5\,\,0.75]     &  [0.75\,\,1.0]    \\
$\mathrm{7}$&  [0.5\,\,0.625]     &  [0.5\,\,0.6250]    \\
$\mathrm{8}$&  [0.625\,\,0.75]     &  [0.5\,\,0.6250]    \\
$\mathrm{9}$&  [0.5\,\,0.6255]     &  [0.625\,\,0.6250]    \\
$\mathrm{10}$&  [0.625\,\,0.75]     &  [0.625\,\,0.750]    \\
 \hline
\end{tabular}
\label{tab:regions}
\end{table}
In Figures~\ref{fig:c1_regular_res_unres} and~\ref{fig:c2_regular_res_unres}, we compare the concentration at the final time $t=t_f$ along the lines $\rm{B-B^{\prime}}$ and $\rm{C-C^{\prime}}$($y=0.5$ in Figure~\ref{fig:unresolved_regular_p}),respectively. We can observe mesh convergence for both the resolved and the unresolved test cases. In particular, while a good agreement is found among all the results related to the unresolved configuration, we observe that the difference among the solutions computed for the resolved test cases progressively reduces with mesh refinement. 
A comparison between the resolved and the unresolved test cases is performed by analyzing both the concentration along lines $B-B^{\prime}$ and $C-C^{\prime}$ and the average concentration in the regions listed in Table~\ref{tab:regions}. The two configurations reveal a good agreement for all the regions except for region $2$ where the solution obtained for the unresolved case $\rm{unres_3}$ is almost half the one computed for the resolved one $\rm{res_3}$. However, we have observed that the concentration in this region progressively decreases by uniformly refining the grid (not shown). Thus, we believe that the differences between the numerical solutions are mainly related to the artificial diffusion introduced by the stabilization which prevents the concentration to become zero.

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_res_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_unres_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_tot}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}


\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/pressure_u_r}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/cm_res_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{fig/regular/cm_ures_comp}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/regular/cm_res_vs_ures_1}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/regular/cm_res_vs_ures_2}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm]{fig/regular/cm_res_vs_ures_3}
\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
\label{fig:regular_p1_res_unres}
\end{figure}

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures/fig_single_4}
%\includegraphics[width=8cm]{figures/fig_mesh_2}
%\caption{Concentration profiles for the benchmark \textit{single2d}  at final time along the fracture $(50\,;\,-30\,;\,0), (-50\,;\,30\,;\,0)\,m$ for the test case 4.}
%\label{fig:figure_c3_bench1}
%\end{figure}

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_3.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_4.eps}
%\caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the lines $x=0.5$ and $y=0.7$ for different conformed-mesh size}
%\label{fig:regular_p1_unres}
%\end{figure}

\clearpage

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_1.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_1.eps}
%\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
%\label{fig:regular_p1_res_unres}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_2.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_2.eps}
%\caption{Pressure along the line $B-B^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases. (Conductive)}
%\label{fig:regular_p1_res_unres}
%\end{figure}
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/fig_1}
%\includegraphics[width=6cm]{figures_new/regular/fig_2}
%\caption{Comparison among the pressure profiles along the lines $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for test cases $res_3$, $unres_3$, and the reference solution (Conductive).}
%\label{fig:regular_p1_p2_comp}
%\end{figure}

\clearpage

%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=3.8cm]{figures/regular/RegularConfP1.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularAMRp1.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularVerticalLine}
%\caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $x=0.5$ for different conformed-mesh size}
%\label{fig:figure_conf_bench2}
%\end{figure}

% \begin{figure}[hbt!]
% \centering
% \includegraphics[width=8cm]{figures/RegularAmr}
% \caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $x=0.5$ for different AMR-mesh size}
% \label{fig:figure_amr_bench2}
% \end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=3.8cm]{figures/regular/RegularConfp2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularAMRp2.eps}
%\includegraphics[width=3.8cm]{figures/regular/RegularHorizontalLine.png}
%\caption{Benchmark 2 with conductive fractures: comparison of hydraulic pressure values along the line $y=0.7$}
%\label{fig:figure_p1_bench2}
%\end{figure}


%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_3.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_5.eps}
%\caption{Concentration at final time $t=0.5~[s]$ along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
%\label{fig:c1_regular_res_unres}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/resolved/fig_4.eps}
%\includegraphics[width=6cm]{figures_new/regular/unresolved/fig_6.eps}
%\caption{Comparison among the concentration profiles along the lines $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for test cases $res_3$, $unres_3$ (Conductive).}
%\label{fig:c1_c2_regular_res_unres}
%\end{figure}
%
%
%
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular/fig_3}
%\includegraphics[width=6cm]{figures_new/regular/fig_4}
%\caption{Concentration at final time $t=0.5~[s]$ along the line $B-B^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases (Conductive).}
%\label{fig:c2_regular_res_unres}
%\end{figure}
%
%
%
%
%\begin{figure}[hbt!]
%\hspace{-0.8cm}\includegraphics[width=12cm]{figures_new/regular/fig_5}
%\caption{Average concentration in the regions defined in~\ref{tab:regions} over time (Conductive).}
%\label{fig:figure_c_bench2}
%\end{figure}
%
%
%\subsubsection{Blocking fracture network}
%We now present the numerical results obtained for the blocking fracture network. In particular, we focus on the comparison between the numerical results obtained by solving the flow problem on the resolved and the unresolved meshed reported in Table~\ref{tab:mesh_2}. As an example, the pressure distribution is shown in Figure~\ref{fig:regular_blocking_p} where 
%one may observe the pressure discontinuities induced by the low fracture permeability.
%Figures~\ref{fig:regular_res_unres_p_blocking} and ~\ref{fig:comparison_res_unres_p_blocking} depict the pressure profile along the line $\rm{A-A^{\prime}}$, with coordinated $A=(0.1,0,0)$ and $A^{\prime}=(1.0,0.9,0)$ . Again a good agreement is found among all the numerical solutions.
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=7cm]{figures_new/regular_p_blocking_2}
%\caption{Pressure distribution for unresolved test case $\rm{unres_3}$ (Blocking).}
%\label{fig:regular_blocking_p}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=6cm]{figures_new/regular_blocking/resolved/fig_1}
%\includegraphics[width=6cm]{figures_new/regular_blocking/unresolved/fig_1}
%\caption{Pressure along the line $A-A^{\prime}$ for the resolved (Left) and the unresolved (Right) test cases. (Blocking)}
%\label{fig:regular_res_unres_p_blocking}
%\end{figure}
%
%\begin{figure}[hbt!]
%\centering
%\includegraphics[width=7cm]{figures_new/regular_blocking/fig_1}
%\caption{Comparison among the pressure profiles along the line $\rm{A-A^{\prime}}$ for test cases $res_3$, $unres_3$, and the reference solution (Blocking).}
%\label{fig:comparison_res_unres_p_blocking}
%\end{figure}



\begin{table}[ht!]
\caption{Parameters Setting for conductivity and porosity}
\centering
\begin{tabular}{ |p{4cm}||p{1cm}|}
 \hline
 \multicolumn{2}{|c|}{Parameters Values} \\
 \hline
matrix conductivity $K_{M1}$    &  $1$ \\
fracture conductivity $K_{F}$     &   $10^{4}$ \\
matrix porosity$\phi_{M1}$    & $0.2 $ \\
fracture porosity$\phi_{F}$      & $0.2$\\
 \hline
\end{tabular}
\label{tab:param_3}
\end{table}



\begin{figure}[hbt!]
\centering
\includegraphics[width=10cm]{figures_new/small_features/small_feat_geo}
\caption{Geometry Setup and Boundary Conditions (top). Fracture Network (Bottom).}
\label{fig:small_feat_p_1_2_res}
\end{figure}



\begin{figure}
\centering
\subfloat[Unresolved case 1]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea1grid.png}}
\subfloat[Unresolved case 2]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea2grid.png}}\\
\subfloat[Unresolved case 3]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea4grid.png}}
\subfloat[Unresolved case 4]{\includegraphics[width= 2.0in]{figures_new/small_features/smafea6grid.png}}
\label{mesh_unreolved}
\end{figure}

\begin{table}[ht]
\caption{Mesh Setting}
\centering
\begin{tabular}{ |p{2cm}||p{2cm}|p{2cm}|p{2cm}|  }
 \hline
 \multicolumn{4}{|c|}{Resolved Mesh} \\
 \hline
          &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# layers\\
 \hline
$\mathrm{res_1}$    &     3823   &     19964 & 1\\ 
$\mathrm{res_2}$    &      28519   &     159712  & 2\\
$\mathrm{res_3}$    &      220325   &    1277696  &  3\\
$\mathrm{res_4}$    &   1732172   &    10221568 &  4\\
 \hline
 \multicolumn{4}{|c|}{Unresolved Mesh} \\
  \hline
          &\bfseries \# nodes    & \bfseries \# elem& \bfseries \# layers\\
 \hline
$\mathrm{unres_1}$    &      667672  &      560290 & ~1\\ 
$\mathrm{unres_2}$    &           964549   &      933120  & ~2\\
$\mathrm{unres_3}$    &     18634058   &    16727570  &  ~3\\
$\mathrm{unres_4}$    &     90026102  &     84703700 &  ~6\\
 \hline
\end{tabular}
\label{tab:mesh_3}
\end{table}

\subsection{Small Features}
%\begin{enumerate}
%\item  we observe a slow convergence for both the resolved and the unresolved case. Jump in the values used for the constitutive parameters and  for the neumann boundary conditions  affect the regularity of the solution and (The regularity of  the solution is less than $H^2$). A priori, both these issues reduce the convergence rate of the FE method, as the sol must be at least $p-1$ in order to converge with order $p$. The reduction of the convergence rate  due to the jump in the parameters can be avoided with a mesh that resolves the boundary of the discontinuity. In this case, we may get the expected order of convergence. Instead, the problem related to the  discontinuities in the values used for the boundary conditions can not be avoided in any way with the standard continuous fe methods. Possible solutions are to use methods GFEM or multiscale that add special functions to the type of discontinuity, or try to make AMR near the region where boundary conditions changes occur. (Maybe we can mention this also for the regular case)
%\item for the plots over region one may notice a good agreement between the resolved and the unresolved case. Can we say the same also for the pressure?
%\end{enumerate}

\begin{figure}
\centering
\subfloat[a)Spatial  distribution of the pressure]{\includegraphics[width=10cm]{figures_new/small_features/p_small_feat_1}}\\
\subfloat[b) Spatial  distribution of the pressure in the planes $x=0.5$ and $z=0.5$ where line $A-A^{\prime}$ and $B-B^{\prime}$ lie]{\includegraphics[width=10cm]{figures_new/small_features/p_small_feat_2}}
\label{fig:small_feat_p_unres}
\end{figure}




\begin{figure}
\centering
\includegraphics[width=6cm]{figures_new/small_features/resolved/fig_1}
\includegraphics[width=6cm]{figures_new/small_features/resolved/fig_2}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_p_1_2_res}
\end{figure}


\begin{figure}[hbt!]
\centering
\includegraphics[width=6cm]{figures_new/small_features/unresolved/fig_1}
\includegraphics[width=6cm]{figures_new/small_features/unresolved/fig_2}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_p_1_2_unres}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=6cm]{figures_new/small_features/fig_1}
\includegraphics[width=6cm]{figures_new/small_features/fig_2}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_comp}
\end{figure}
\begin{figure}[hbt!]
\hspace{-0.8cm}\includegraphics[width=14cm]{figures_new/small_features/fig_3}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:small_feat_conc}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=8cm]{figures_new/small_features/c_small_feat}
\caption{Concentration at last time step.}
\label{fig:small_feat_c_ures}
\end{figure}




This benchmark allows for testing the accuracy of the proposed method in the presence of small geometric features. The matrix background is a box $M=(0\,;\,1)\times(0\,;\,2.25)\times(0\,;\,1)\, m$, containing eight fractures.
These are defined by their vertexes and described in~\cite{flemisch2018benchmarks}. The inlet and the outlet are defined as follows: $\partial \Omega_{in}=(0\,;\,1)\times(0)\times(1/3\,;\,2/3)\,m$, $\partial \Omega_{out,1}=(0\,;\,1)\times(2.25)\times(0\,;\,1/3)\,m$,
$\partial \Omega_{out,2}=(0\,;\,1)\times(2.25)\times(1/3\,;\,2/3)\,m$. 

For the flow problem, a uniform inflow on the inlet such that $\int_{\partial \Omega_{in}}\mathbf{u}\cdot \mathbf{n}\,d\gamma=-1/3$, whereas homogeneous Dirichlet boundary conditions are applied on the outlet $\partial \Omega_{out}=\partial \Omega_{out,1}\cup\partial \Omega_{out,2}$. No flow (Neumann) boundary conditions are set on the other boundaries. 

For the transport problem, a Dirichlet boundary condition is imposed on the inlet: $c_{in}=1.0\,m$.
The overall simulation time is set equal to $t_f=10^{2}\,s$ while the time step is set equal to$dt=0.01$.  All the material parameters are summarized in table~\ref{tab:param_3}:


Table ~\ref{tab:mesh_1} lists the number nodes and elements for all performed test cases. As an example, in Figures \ref{mesh_unreolved} and ~\ref{p_small_feat_2} we show the meshes obtained by adopting the adaptive refinement to model the fracture network geometry for all the unresolved test cases reported in Table ~\ref{tab:mesh_1}, and the spatial distribution obtained for test case $\rm{unres}_3$ . In particular ~\ref{p_small_feat_2} b) depicts the spatial distribution of the pressure at planes $x=0.5$ and $z=0.5$ and the extreme points $A=(0.5,\,1.1,\,0)-A^{\prime}=(0.5,\,1.1,\,1)$, and $B=(0,\,2.15,\,0.5)-B^{\prime}=(1,\,2.15,\,0.5)$ of the lines along which the pressure profiles are analized.

Figures~\ref{fig:small_feat_p_1_2_res} and ~\ref{fig:small_feat_p_1_2_unres} depict the pressure profile along the line $A-A^{\prime}$ and $B-B^{\prime}$, for the resolved and the unresolved test cases reported in Table~\ref{tab:mesh_3}. 
We observe that the accuracy of the solution strongly depends on the mesh size for all the performed numerical simulations. 
Figure~\ref{fig:small_feat_comp} shows a comparison between the test cases $\rm{res_4}$ and $\rm{ures_4}$. Small discrepancies can be appreciated since mesh converge was observed neither for the unresolved nor for the resolved test case.

In this regard, it is worth mentioning that the jumps in the values used for the constitutive parameters and the Neumann boundary conditions affect the regularity of the solution. A priori, both these issues reduce the convergence rate of the FE method, as the sol must be at least $p-1$ to converge with order $p$. The reduction of the convergence rate due to the jump in the parameters can be avoided with a mesh that resolves the boundary of the discontinuity. In this case, we may get the expected order of convergence. Instead, the problem related to the discontinuities in the values used for the boundary conditions can not be avoided in any way with the standard continuous Finite Element  Methods. Possible solutions are to use methods GFEM or multiscale that add special functions to the type of discontinuity or try to make AMR near the region where boundary conditions changes occur.
Finally, we analyze the average concentration in each fracture and plot the results in Figure~\ref{fig:small_feat_conc} which reveals a good agreement between the test cases $\rm{res_4}$ and $\rm{ures_4}$. Indeed, as one may observe
figures~\ref{fig:small_feat_p_1_2_res} and ~\ref{fig:small_feat_p_1_2_unres}, the progressive refinement performed to solve for the flow problem, produces as the main effect the sum of a constant to the coarsest solution. Hence, even though the values of the pressure field increase,  the computation of the corresponding gradient, and consequently of the velocity field, will produce similar results.







\subsection{Hydrocoin}
%\begin{enumerate}
%\item good agreement between unresolved and the reference solution
%\end{enumerate}
This flow problem was presented within the international Hydrocoin project, (Swedish Nuclear Power Inspectorate (SKI) and proposed as benchmark for both hybrid and equi-dimensional models in~\cite{flemisch2018benchmarks}. Concerning the boundary conditions,  a piezometric head is imposed on the top boundary of the domain, whereas  no  flow (Neumann) boundary conditions are set on the other boundaries. We only consider the unresolved test case consisting of $12683$ elements and $10938$ nodes and compare the corresponding solution for the pressure with the reference  solution obtained by a standard FV method on a continuous fracture model and computed on a grid with $3 527 296$
elements and $3 813 249$ nodes ~\cite{flemisch2018benchmarks}. 
\begin{table}[htb!]
\caption{Parameters Setting for conductivity and porosity}
\centering
\begin{tabular}{ |p{4cm}||p{1cm}|}
 \hline
 \multicolumn{2}{|c|}{Parameters Values} \\
 \hline
matrix conductivity $K_{M}$    &  $10^{-8}$ \\
fracture conductivity $K_{F}$    &  $10^{-6}$ \\
 \hline
\end{tabular}
\label{tab:param_1}
\end{table}

\begin{figure}[hbt!]
\centering
\includegraphics[width=13cm ]{figures_new/hydro}
\caption{Benchmark 1. Locally refined mesh with Ndof equato to 259600 (AMR$_5$). Fractures are represent by means an AME techniques,}
\label{fig:setup_hydro}
\end{figure}
\begin{figure}[ht]
\centering
\includegraphics[width=7cm]{figures_new/hydrocoin/fig}
\caption{Pressure profiles for  the benchmark \textit{hydrocoin} along the line $A-A^{\prime}$ }
\label{fig:hydro_p}
\end{figure}


Figure~\ref{fig:setup_hydro} shows the pressure distribution and the extreme points of  $A=(0\,;\,-200\,;\,0)$ and $A^{\prime}=(1600\,;\,-200\,;\,0)$ of the line along which the pressure is analyzed.  In Figure~\ref{fig:hydro_p}, we observe a good agreement between the numerical results obtained for the unresolved test case and the reference solution.


\subsection{Realistic}

In this last test case, we consider a real set of fractures from an interpreted outcrop in the Sotra island, near Bergen in Norway. The set comprises
64 fractures grouped in 13 different connected networks, ranging from isolated fractures up to tens of fractures each. In the interpretation process, two fractures are composed of more than one segment. The size of the domain is $700\,m \times 600 \,m$ with uniform matrix permeability $K_m = 10$. For simplicity, all the fractures have the same scalar permeability $K_f=10^{-6}$. Concerning the boundary conditions, we consider homogeneous Neumann boundary conditions (no flow) on the top and bottom side, a pressure $P= 1013250\,[Pa]$ is applied on the left side, and pressure $P=0\,[Pa]$ on the right side of the domain.
In Figure~\ref{fig:realistic_line_1} we analize the mesh converge by analyze the pressure along the lines $\rm{A-A^{\prime}}$ and $\rm{B-B^{\prime}}$ for all the unresolved test cases reported in Table~\textbf{add table}.
While we observe that all the pressure profiles show similar behavior, relevant differences are found in the pressure distribution reported in Figure~\ref{fig:realistic_pressure} where a similar pattern is only observed for the test cases $\rm{unres_3}$ and $\rm{unres_4}$.
Figure~\ref{fig:realistic_line_1} shows a comparison between our numerical results and those obtained with the numerical methods presented in ~\cite{flemisch2018benchmarks}. Again a good agreement is found among all the profiles. 

\begin{figure}
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh0.pdf}}
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh3.pdf}}\\
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh4.pdf}}
\subfloat[caption]{\includegraphics[width= 2in]{figures_new/realistic/realisticMesh6.pdf}}
\end{figure}



\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm]{figures_new/realistic/convergence}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:realistic_line_1}
\end{figure}



\begin{figure}[hbt!]
\centering
\includegraphics[width=12cm]{figures_new/realistic/fig_realistic_p_tot}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:realistic_pressure}
\end{figure}


\begin{figure}[hbt!]
\centering
\includegraphics[width=7cm]{figures_new/realistic/comparison}
\caption{Pressure profiles for  the benchmark \textit{Small features} along the line $(0.5\,;\,1.1\,;\,0), (0.5\,;\,1.1\,;\,1)\,m$ }
\label{fig:realistic_line_1}

\end{figure}



\newpage

%\printbibliography




